On the Relative Usefulness of Fireballs

In CSL-LICS 2014, Accattoli and Dal Lago showed that there is an implementation of the ordinary (i.e. strong, pure, call-by-name) $\lambda$-calculus into models like RAM machines which is polynomial in the number of $\beta$-steps, answering a long-standing question. The key ingredient was the use of a calculus with useful sharing, a new notion whose complexity was shown to be polynomial, but whose implementation was not explored. This paper, meant to be complementary, studies useful sharing in a call-by-value scenario and from a practical point of view. We introduce the Fireball Calculus, a natural extension of call-by-value to open terms for which the problem is as hard as for the ordinary lambda-calculus. We present three results. First, we adapt the solution of Accattoli and Dal Lago, improving the meta-theory of useful sharing. Then, we refine the picture by introducing the GLAMoUr, a simple abstract machine implementing the Fireball Calculus extended with useful sharing. Its key feature is that usefulness of a step is tested---surprisingly---in constant time. Third, we provide a further optimization that leads to an implementation having only a linear overhead with respect to the number of $\beta$-steps.

==> explicit-machine.tex <==
% !TEX root = main.tex
\section{An Inefficient Distillery: the \GLAM\ Machine}\label{sect:glam}
\begin{atend}\section{Proofs Omitted From \refsect{glam}\\ (An Inefficient Distillery: the \GLAM\ Machine)}\end{atend}
\begin{atend}
The aim of this section is to prove \refth{glam-refl-distillation}, \ie\ that 
$(\GLAM,\togens, \eqstruct, \decodefun)$ is a reflective explicit distillery.

\end{atend}

In this section we introduce the \GLAM\ machine and show that it distills to the \ShFC. The distillery is inefficient, because \ShFC\ suffers of size explosion, but it is a good case study to present distilleries before the optimizations. Moreover, it allows to show an unexpected fact: while adding useful sharing to the calculus will be a quite tricky and technical affair (\refsect{useful}), adding usefulness to the \GLAM\ will be surprisingly simple (\refsect{glamour}), and yet tests of usefulness will only require costant time.

The machine of this section is the Global LAM (\GLAM). The name is due to a similar machine, based on \emph{local} environments, introduced in \cite{DBLP:conf/icfp/AccattoliBM14} and called LAM---standing for Leroy Abstract Machine. The \GLAM\ differs from the LAM in two respects: 1) it uses \emph{global} rather than local environments, and 2) it has an additional rule to handle constructors. 

\paragraph*{Data-Structures} at the machine level, \emph{terms} are replaced by \emph{codes}, \ie\ terms not considered up to $\alpha$-equivalence. To distinguish codes from terms, we over-line codes like in $\code$.

States (noted $\state,\statetwo,\ldots$) of the abstract machine are made out of a \emph{context dump} $\dump$, a \emph{code} $\tm$, an \emph{argument stack} $\stack$, and a global environment $\genv$, defined by the grammars in \reftab{transitions}. To save space, sometimes we write $\esub\var{\code}\genv$ for $\esub\var{\code}\cons\genv$. Note that stacks may contain pairs $\pair{\code}{\stack}$ of a code and a stack, used to code the application of $\code$ to the stack $\stack$. We choose this representation to implement commutative rules in constant time.

\paragraph*{The Machine} the machine transitions are given in \reftab{explicit-transitions}. Note that the multiplicative one $\tomachsm$ puts a new entry in the environment, while the exponential one $\tomachse$ performs a clashing-avoiding substitution from the environment. The idea is that the principal transitions $\tomachsm$ and $\tomachse$ implement $\togensm$ and $\togense$ while the commutative transitions $\tomachcone$, $\tomachctwo$, and $\tomachcthree$ locate and
expose the next redex following a right-to-left strategy.

The commutative rule $\tomachcone$ forces evaluation to be right-to-left on applications: the machine processes first the argument $\codetwo$, saving the left sub term $\code$ on the dump together with its current stack $\stack$.
The role of $\tomachctwo$ and $\tomachcthree$ is to backtrack to the saved sub-term. Indeed, when the argument, \ie\ the current code, is finally put in normal form, encoded by
a \emph{stack item} $\stackitem$, the stack item is pushed on the stack, and the machine backtracks to the pair on the dump.

\paragraph*{The Distillery} machines start an execution on \emph{initial states} defined as $ \glamst\stempty\code\stempty\stempty$, \ie\ obtained by taking the term, seen now as the code $\code$, and setting to
$\stempty$ the other machine components. A state represents a term---given by the code---and an evaluation context, that for the \GLAM\ is obtained by decoding $\dump$, $\stack$, and $\genv$. The decoding $\decodefun$ (or distillation) function is defined in \reftab{explicit-transitions}.
Note that stacks are decoded to contest in postfix notation for plugging. To improve readability, when we will decode machines,
we will denote $\wctxp\tm$ with $\ctxholep\tm\wctx$, if the component
occurs on the right of $\tm$ in the machine representation.



A machine state is \emph{closed} when all free variables in any component of the state are bound
in $\genv$ or, equivalently, when $\decode{\state}$ is closed in the usual sense.
It is \emph{well-named} when all variables bound in the state are
distinct. We require well-namedness as a machine invariant to allow
every environment entry $\esub\var{\code}$ to be global (i.e. to bind $\var$
everywhere in the machine state). From now on, the initial state associated to a term $\tm$ has as code the term obtained $\alpha$-converting $\tm$ to make it well-named.


For every machine  we will have invariants, in order to prove the properties of a distillery. They are always proved by induction over the length of the execution, by a simple inspection of the transitions. For the \GLAM:

\begin{lemma}[GLAM Invariants]\label{l:GLAMInvariants}
	Let $\state = (\dump,\tmtwo,\stack,\genv)$ be a state reachable from an initial code $\code$. Then:
	\begin{enumerate}
		\item \label{p:GLAMInvariants-one}\emph{Closure}: $\state$ is closed and well-named;
		\item \label{p:GLAMInvariants-two}\emph{Value}: values in components of $\state$ are sub-terms of $\code$;
		\item \label{p:GLAMInvariants-three}\emph{\Fireball}: every term in $\stack$, in $\genv$, and in every stack in $\dump$ is a \fireball;
		\item \label{p:GLAMInvariants-four}\emph{Contextual Decoding}: $\decgenv$, $\decdump$, $\decstack$, and $\evctx_\state$ are evaluation contexts;
		%\item \label{p:GLAMInvariants-five}\emph{Environment Size}: the length of the global environment $\genv$ is bound by $\sizem\exec$.
	\end{enumerate}
\end{lemma}

\begin{proofatend}
by induction over the length of the execution.
The base case holds because $\code$ is initial.
The inductive step is by cases over the kind of transition.
All the verifications are trivial inspections of the transition.
\end{proofatend}

\begin{atend}
\input{\proofspath/explicit-glam-distillation}
\end{atend}

The invariants are used to prove the following theorem.

\begin{theorem}[\GLAM\ Distillation]\label{th:glam-refl-distillation}
	$(\mbox{\GLAM},\togens, \eqstruct, \decodefun)$ is a reflective explicit distillery. In particular, let $\state$ be a reachable state reachable:
		\begin{enumerate}
		\item \emph{Commutative}: if $\state\tomachcp{_{1,2,3}}\statetwo$ then $\decode\state=\decode\statetwo$;
		\item \emph{Multiplicative}: if $\state\tomachsm\statetwo$ then $\decode\state\togensm\eqstruct\decode\statetwo$;
		\item \emph{Exponential}: if $\state\tomachse\statetwo$ then $\decode\state\togense\decode\statetwo$.
	\end{enumerate}
\end{theorem}
\begin{proofatend}
it follows from \reflemma{glam-distillation} and \reflemma{progress}.
\end{proofatend}

Since the \ShFC\ suffers of size-explosion, an exponential step (and thus an exponential transition) may duplicate a subterm that is exponentially bigger than the input. Then $(\mbox{\GLAM},\togens, \eqstruct, \decodefun)$ does not satisfy bilinearity, for which \claudio{every exponential transition has to have linear complexity in the size of the input}.


==> high-level.tex <==
% !TEX root = main.tex
% !TEX root = main.tex
\section{Two Levels Implementation}
Here we explain how the the small-step strategy $\tof$ of the \FC\ is implemented by a micro-step strategy $\togen$. We are looking for an appropriate strategy $\calculus$ with ES which is polynomially related to both $\tof$ and an abstract machine. Then we need two theorems:
\begin{enumerate}
\item 
  \emph{High-Level Implementation}: $\tof$ terminates iff
  $\calculus$ terminates. Moreover, $\tof$ is implemented by $\calculus$
  with only a polynomial overhead. Namely, $\tm\calculus^k\tmtwo$ iff
  $\tm\tof^h\unf{\tmtwo}$ with $k$ polynomial in $h$;
\item 
  \emph{Low-Level Implementation}: $\calculus$ is implemented on an abstract machine with an overhead in time which is polynomial in both $k$ and the size of $\tm$.
\end{enumerate}
We will actually be more accurate, giving linear or quadratic bounds, but this is the general setting.

\subsection{High-Level Implementation}
First, terminology and notations. \emph{Derivations} $\deriv,\derivtwo,\ldots$ are sequences of rewriting steps. With $\size\deriv$, $\sizem\deriv$, and $\sizee\deriv$ we denote respectively the length, the number of multiplicative, and exponential steps of $\deriv$. 

\begin{definition}\label{def:hlis}
Let $\tof$ be a deterministic strategy on \FC-terms and $\calculus$ a
deterministic strategy for terms with ES. The pair $(\tof,\calculus)$ is a
\deff{high-level implementation system} if whenever $\tm$ is a
$\l$-term and $\deriv:\tm\calculus^*\tmtwo$ then:
\begin{enumerate}
  \item 
    \emph{Normal Form}: if $\tmtwo$ is a $\calculus$-normal form then
    $\unf{\tmtwo}$ is a $\tof$-normal form.
  \item 
    \emph{Projection}: $\unf{\deriv}:\unf{\tm}\tof^*\unf{\tmtwo}$ and
    $\size{\unf{\deriv}}=\sizem\deriv$.
    \end{enumerate}
Moreover, it is 
\begin{enumerate}
	\item \emph{locally bounded}: if the length of a sequence of substitution $\esym$-steps from $\tmtwo$ is linear in the number $\sizem\deriv$ of $\msym$-steps in $\deriv$;
	\item \emph{globally bounded}: if $\sizee\deriv$ is linear in $\sizem\deriv$.
\end{enumerate}
\end{definition}

The normal form and projection properties address the
\emph{qualitative} part, \ie\
the part about termination. The normal form property guarantees that
$\calculus$ does not stop prematurely, so that when $\calculus$ terminates
$\tof$ cannot keep going. The projection property guarantees that
termination of $\tof$ implies termination of $\calculus$. The two
properties actually state a stronger fact: \emph{$\tof$ steps can
  be identified with the $\togenm$-steps of the $\calculus$ strategy}.

The local and global bounds allow to bound the overhead introduced by the \ShFC{} wrt the \FC, because by relating $\togenm$ and $\togene$ steps, they relate $\size\deriv$ and $\size{\unf\deriv}$, since $\tof$ and $\togenm$ steps can be identified.

The high-level part can now be proved abstractly.
\begin{theorem}[High-Level Implementation]\label{thm:hlithm}
  Let $\tm$ be an ordinary $\l$-term and $(\tof,\calculus)$ a
  high-level implementation system.
  \begin{enumerate}
	  \item \emph{Normalization}: $\tm$ is $\tof$-normalizing iff it is $\calculus$-normalizing.
	  \item \emph{Projection}: if $\deriv:\tm\calculus^*\tmtwo$ then
    $\unf{\deriv}:\tm\tof^*\unf{\tmtwo}$.
  \end{enumerate}
  Moreover, the overhead of $\calculus$ is, depending on the system:
  \begin{enumerate}
	\item \emph{locally bounded}: quadratic, \ie\ $\size\deriv=O(\size{\unf{\deriv}}^2)$.
	\item \emph{globally bounded}: linear, \ie\ $\size\deriv=O(\size{\unf{\deriv}})$.
\end{enumerate}    
\end{theorem}

\begin{proofatend}
The proof is a minimal variation over the proof of Theorem 4.2, page 4, in \cite{DBLP:conf/csl/AccattoliL14}. Essentially we merged the trace and syntactic bound properties of that statement into our locally bound property. Note that for the global bound there is nothing to prove, it follows from the the hypothesis itself and projection.
\end{proofatend}
\noindent For the low-level part, in contrast to \cite{DBLP:conf/csl/AccattoliL14}, we rely on abstract machines, introduced in the next section.

Let us see our framework at work. We have the following result: 

\begin{theorem}\label{thm:explicithlis}
	$(\tof,\togens)$ is a high-level implementation system.
\end{theorem}
\begin{proofatend}
Immediate from \refcoro{es-closed-determ} and
\reflemma{unfolding-steps}.
\end{proofatend}

Note the absence of complexity bounds. In fact, $(\tof,\togens)$ is not even locally bounded. Let $\tm^n$ here be defined by $\tm^1 = \tm$ and $\tm^{n+1} = \tm^{n} \tm$, and $\tmtwo_n \defeq (\la\var\var^n) \gconst$. Then $\deriv:\tmtwo_n \togenm\togene^n \gconst^n\esub\var\gconst$ is a counter-example to local boundedness. Moreover, the \ShFC\ also suffers of size explosion, \ie\ implementing a single step may take exponential time. In \refsect{useful} the introduction of useful sharing will solve these issues.

%
%\begin{definition}
%\label{def:mech}
%A strategy $\calculus$ on \lsc\ terms is \deff{mechanisable} if given a
%derivation $\deriv:\tm\calculus^*\tmtwo$:
%\begin{enumerate}
%\item 
%  \emph{Subterm}: the terms duplicated along $\deriv$ are subterms of
%  $\tm$.
%\item 
%  \emph{Selection}: the search of the next $\calculus$ redex to reduce in
%  $\tmtwo$ takes polynomial time in $\size\tmtwo$.
%\end{enumerate}
%\end{definition}
%The \emph{subterm property}---essentially---guarantees
%that any step has a linear cost in the size of the initial term, the
%fundamental parameter for complexity; it will be discussed in more
%detail in \refsect{standard}. At first sight the \emph{selection
%  property} is always trivially verified: finding a redex in $\tmtwo$
%takes time linear in $\size\tmtwo$. However, our strategy for ES will
%reduce only redexes satisfying a side-condition whose na\"ive
%verification is exponential in $\size\tmtwo$. Then one has to be sure
%that such a computation can be done in polynomial time.
%
%\begin{theorem}[Low-Level Implementation]
%  Let $\calculus$ be a mechanisable strategy. % Then there is an algorithm  that on input $\tm$ and $k$ outputs $\strp{\calculus}{k}{\tm}$, and
%  which works in time polynomial in $k$ and $\size\tm$.
%\end{theorem}
%\begin{IEEEproof}
%  By the subterm property, implementing one step takes time polynomial
%  (if not linear) in $\size\tm$. An immediate consequence of the
%  subterm property is the \emph{no size explosion property}, \ie\ that
%  $\size\tmtwo\leq(k+1)\cdot\size\tm$. By the selection property
%  selecting the next redex takes time polynomial in $\size\tmtwo$,
%  that by the no size explosion property is polynomial in $k$ and
%  $\size\tm$. The composition of polynomials is again a polynomial,
%  and so selecting the redex takes time polynomial in $k$ and
%  $\size\tm$. Hence, the reduction can be implemented in polynomial  time.
%\end{IEEEproof}
%
%In \cite{DBLP:conf/rta/AccattoliL12}, we proved that \emph{head
%  reduction} and \emph{linear head reduction} form a high-level
%implementation system and that linear head reduction is mechanisable,
%even if we did not use such a terminology, nor were we aware of the
%presented abstract scheme. In order to extend such a result to normal
%forms we need to replace head reduction with a normalising strategy
%(\ie\ a strategy reaching the $\beta$-normal form, if any).
%
%One candidate for $\tof$ is the \lo\ strategy $\toblo$. Such a
%choice is natural, as $\toblo$ is normalising, it produces standard
%derivations, and it is an iteration of head reduction. What is left to
%do, then, is to find a strategy $\calculus$ for ES, which is both
%mechanisable and a high-level implementation of
%$\toblo$. Unfortunately, the linear \lo\ strategy, noted $\tollo$
%and first defined in \cite{non-standard-preprint}, is mechanisable but
%the pair $(\toblo,\tollo)$ is not a high-level implementation system.
%
%In general, mechanisable strategies are not hard to find. As we will
%show in \refsect{standard}, the whole class of \emph{standard}
%derivations for ES has the subterm property. In particular, the linear
%strategy $\tollo$---which is standard---enjoys all the other
%properties \emph{but} for the syntactic bound property.
%
%Such a problem will be solved by \lo\ \emph{useful} derivations, to be
%introduced in \refsect{useful}, that will be shown to be both
%mechanisable and a high-level implementation of $\toblo$. Useful
%derivations avoid those substitution steps that only explicit the
%normal form without contributing to explicit $\beta/\db$-redexes
%(that, by the projection property, can be identified). \lo\ useful
%derivations will have all the nice properties of \lo\ derivations and
%moreover will stop on shared, minimal representations of normal forms,
%solving the problem with linear \lo\ derivations.
%
%Let us point out that our analysis would be vacuous without evidence
%that useful normal forms are a reasonable representation of
%$\l$-terms. In other words, we must be sure that ES do not hide (too
%much of) the inherent difficulty of reducing $\lambda$-terms under the
%carpet of sharing. In~\cite{DBLP:conf/rta/AccattoliL12}, we solved
%this issue by providing an efficient algorithm for checking the
%equality of any two \lsc\ terms---thus in particular of useful normal
%forms---without computing their unfoldings (that otherwise would
%reintroduce an exponential blow-up). Some further discussion can be
%found in Sect.~\ref{sect:properties}.



==> interlude-contexts.tex <==
% !TEX root = main.tex

\section{Interlude I:\\ Formalities about Contexts}
\label{sect:contexts}
The dynamics of explicit substitutions is defined using (one-hole) contexts, formally defined here. \emph{Weak contexts} subsume all the kinds of context in the paper, and are defined by
\begin{center}$\begin{array}{lllllllllllll}
	\wctx,\wctxtwo 		& \grameq & \ctxhole\mid \tm\wctx\mid \wctx\tm \mid \wctx\esub\var\tm \mid \tm\esub\var\wctx
\end{array}$\end{center}
The plugging $\wctxp\tm$ of a term $\tm$ into a context $\wctx$ is defined as
$\ctxhole\ctxholep\tm\defeq\tm$, $(\l\var.\wctx)\ctxholep\tm \defeq
\l\var.(\wctx\ctxholep\tm)$, and so on. As usual, plugging in a
context can capture variables,
\eg\ $((\ctxhole\vartwo)\esub\vartwo\tm)\ctxholep\vartwo =
(\vartwo\vartwo)\esub\vartwo\tm$. The plugging $\wctxp\wctxtwo$ of a
context $\wctxtwo$ into a context $\wctx$ is defined analogously. Since all kinds of context we will deal with will be weak, the definition of plugging applies uniformly to all of them.

To improve readability, when we will decode machines,
we will denote $\wctxp\tm$ with $\ctxholep\tm\wctx$, if the component
occurs on the right of $\tm$ in the machine representation.

A special and frequently used class of contexts is that of
\emph{substitution contexts} $\sctx\grameq\ctxhole\mid
\sctx\esub{\var}{\tm}$.


==> interlude-unfolding.tex <==
% !TEX root = main.tex
\section{Interlude: Relative Unfoldings}
\label{sect:rel-unfolding}
\begin{atend}\section{Proofs Omitted From \refsect{rel-unfolding}\\ (Interlude II: Relative Unfoldings)}\end{atend}
Now we define some notions for weak contexts that will be implicitly instantiated to all kind of contexts in the paper. In particular, we define substitution over contexts, and then use it to define the unfolding of a context, and the more general notion of relative unfolding.

\emph{Implicit substitution on weak contexts $\wctx$} is defined by
\begin{center}
$\begin{array}{lllllllllllll}
	\ctxhole\isub\var\tmtwo 			& \defeq & \ctxhole\\
	(\tm \wctx)\isub\var\tmtwo 			& \defeq & \tm\isub\var\tmtwo \wctx\isub\var\tmtwo\\
	(\wctx \tm)\isub\var\tmtwo 			& \defeq & \wctx\isub\var\tmtwo \tm\isub\var\tmtwo\\
	\wctx \esub\vartwo\tm\isub\var\tmtwo	& \defeq & \wctx\isub\var\tmtwo \esub\vartwo{\tm\isub\var\tmtwo}\\
	\tm \esub\vartwo\wctx\isub\var\tmtwo	& \defeq & \tm\isub\var\tmtwo \esub\vartwo{\wctx\isub\var\tmtwo}
\end{array}$
\end{center}

\begin{lemma}
	\label{l:evctx-and-sub-commute}
	Let $\tm$ be a term and $\wctx$ a weak context. Then $\wctxp\tm\isub\var\tmtwo = \wctx\isub\var\tmtwo\ctxholep{\tm\isub\var\tmtwo}$.
\end{lemma}

\begin{proofatend}
	by induction on $\wctx$. 
% 	Cases: \ben{the following proof has to be generalized to weak contexts}
% \begin{enumerate}
% 			\item \emph{Empty context $\sctx = \ctxhole$}. By definition, $\ctxhole\ctxholep\tm\isub\var\tmtwo = \tm\isub\var\tmtwo$ and $\ctxhole\isub\var\tmtwo\ctxholep{\tm\isub\var\tmtwo} = \ctxhole\ctxholep{\tm\isub\var\tmtwo}=\tm\isub\var\tmtwo$.
% 			\item \emph{Application Left $\evctx = \evctxtwo\fire$}. We have
% 			\[\begin{array}{ll}
% 				\evctxp\tm\isub\var\tmtwo & =\\
%                                 (\evctxtwop\tm\fire)\isub\var\tmtwo & =\\
%                                 \evctxtwop\tm\isub\var\tmtwo \fire\isub\var\tmtwo & =_{\ih}\\
%                                 \evctxtwo\isub\var\tmtwo\ctxholep{\tm\isub\var\tmtwo} \fire\isub\var\tmtwo &=\\
%                                 \evctx\isub\var\tmtwo\ctxholep{\tm\isub\var\tmtwo}$$
% 			\end{array}\]
% 			\item \emph{Application Right $\evctx = \tmthree \evctxtwo$}. Follows from the \ih\ as in the application left case.
% 			\item \emph{Substitution $\evctx = \evctxtwo\esub\var\tmthree$}. Follows from the \ih\ as in the application left case.\qedhere
% 		\end{enumerate}
\end{proofatend}

Now, we would like to extend the unfolding to contexts, but in order to do so we have to restrict the notion of context. Indeed, whenever the hole of a context is inside an ES, the unfolding may erase or duplicate the hole, producing a term or a multi-context, which we do not want to. Thus, we turn to (weak) \emph{shallow contexts}, defined by:
$$
\tctx,\tctxtwo,\tctxthree \grameq \ctxhole\mid \tctx \tm \mid\tm\tctx \mid \tctx\esub{\var}{\tm}.
$$
(note the absence of the production $\tm\esub{\var}{\tctx}$).


Now, we define in \reftab{unfolding} \emph{context unfolding} $\unf\tctx$, \emph{unfolding $\relunf\tm\tctx$ of a term $\tm$ relative to a shallow context $\tctx$} and \emph{unfolding $\relunf\tctxtwo\tctx$ of a shallow context $\tctxtwo$ relative to a shallow context $\tctx$}.



Relative unfoldings have a number of properties, summed up in the appendix (page \pageref{l:relunf-properties}). Last, a definition that will be important in the next section.

\begin{definition}[Applicative Context]
\label{def:appl-ctx}
  A shallow context $\tctx$ is \emph{applicative} when its hole is applied to a sub term $\tmtwo$, \ie\ if $\tctx = \tctxtwop{\sctx \tmtwo}$. 
\end{definition}

\begin{atend}
\begin{lemma}[Properties of Relative Unfoldings]
	\label{l:relunf-properties} % \reflemmaeqp{relunf-properties}{four}
	Let $\tm$ and $\tmtwo$ be terms and $\tctx$ be a shallow context.
	\begin{enumerate}
		\item \label{p:relunf-properties-zero} \emph{Commutation}: $\relunf{(\la\var\tm)}\tctx = \relunf{\la\var\tm}\tctx$, 
		$\relunf{(\tm\tmtwo)}\tctx = \relunf\tm\tctx \relunf\tmtwo\tctx$, $\relunf{\tm\isub\var\tmtwo}\tctx = \relunf\tm\tctx \isub\var{\relunf\tmtwo\tctx}$, $\relunf{\tm\isub\var\tmtwo}\tctx = \relunf{\tm\esub\var\tmtwo}\tctx$, 
$\unf\tctx\isub{\var}{\unf\tm} = \unf{\tctx\isub{\var}{\unf\tm}}$, and $\relunf\tm{\tctx\esub\var\tmtwo} = \relunf{\tm\isub\var{\unf\tmtwo}}{\tctx\isub\var{\unf\tmtwo}}$.

		\item \label{p:relunf-properties-one} \emph{Freedom}:
		if $\tctx$ does not capture any free variable of $\tm$ then $\relunf\tm\tctx = \unf\tm$.
		
		\item \label{p:relunf-properties-two} \emph{Relativity}:
		if $\unf\tm =\unf\tmtwo$ then $\relunf\tm\tctx = \relunf\tmtwo\tctx$.
		
		\item \label{p:relunf-properties-three} \emph{Applicativity}:
		if $\tctx$ is applicative then $\unf\tctx$ is applicative.

		\item \label{p:relunf-properties-five} \emph{Splitting}:
		$ \relunf\tm{\tctxp\tctxtwo} = \relunf{\relunf\tm\tctxtwo}{\tctx}$.
		
		\item \label{p:relunf-properties-four} \emph{Factorization}:
		$ \relunf{\tctxtwop\tm}\tctx = \relunf\tctxtwo\tctx \ctxholep{\relunf\tm{\tctxp\tctxtwo}}$, in particular $ \unf{\tctxp\tm} = \unf\tctx \ctxholep{\relunf\tm{\tctx}}$ and $ \relunf{\sctxp\tm}\tctx = \relunf\tm{\tctxp\sctx}$.

	\end{enumerate}
\end{lemma}

%\myproof{
\begin{IEEEproof}
  Routine inductions on $\tctx$ or $\tctxtwo$.
% 	\begin{enumerate}
% 		\item \ben{To do}.
% 	
% 		%%% First Point
% 		\item By induction on $\tctx$. Cases:
% 		\begin{enumerate}
% 			\item \emph{Empty context $\sctx = \ctxhole$}. By definition, $\relunf\tm \ctxhole = \unf\tm$.
% 			\item \emph{Application Left $\tctx = \tctxtwo\fire$}. Follows immediately from the \ih.
% 			\item \emph{Application Right $\tctx = \tmthree \tctxtwo$}. Follows immediately from the \ih.
% 			\item \emph{Substitution $\tctx = \tctxtwo\esub\var\tmthree$}. Then: 
% 			\[\begin{array}{lll}
% 				\relunf\tm{\tctxtwo\esub\var\tmtwo} & =\\
%                                 \relunf\tm\tctxtwo \isub\var{\unf\tmtwo} 	
% 				& =_{\ih}\\
%                                 \unf\tm \isub\var{\unf\tmtwo} & =\\
%                                 \unf\tm
% 			\end{array}\]
% 		where the last step is given by the easy fact that $\fv{\unf\tm} \subseteq \fv\tm$ and by the hypothesis $\var\notin\fv\tm$.
% 		\end{enumerate}
% 
% 		%%% Second Point
% 		\item By induction on $\tctx$. Cases:
% 		\begin{enumerate}
% 			\item \emph{Empty context $\sctx = \ctxhole$}. By definition, $\relunf\tm \ctxhole = \unf\tm$ and $\relunf\tmtwo \ctxhole = \unf\tmtwo$.
% 			\item \emph{Application Left $\tctx = \tctxtwo\fire$}. Then $\relunf\tm\tctx = \relunf\tm {\tctxtwo\fire} = \relunf\tm\tctxtwo =_{\ih} \relunf\tmtwo\tctxtwo = \relunf\tmtwo{\tctxtwo\fire} = \relunf\tmtwo\tctx$.
% 			\item \emph{Application Right $\tctx = \tmthree \tctxtwo$}. Follows immediately from the \ih, as in the previous case.
% 			\item \emph{Substitution $\tctx = \tctxtwo\esub\var\tmthree$}. Then $\relunf\tm\tctx = \relunf\tm {\tctxtwo\esub\var\tmthree} = \relunf\tm\tctxtwo \isub\var{\unf\tmthree}=_{\ih} \relunf\tmtwo\tctxtwo \isub\var{\unf\tmthree} = \relunf\tmtwo{\tctxtwo\esub\var\tmthree} = \relunf\tmtwo\tctx$.
% 		\end{enumerate}
% 
% 		%%% Third Point
% 		\item By induction on $\tctx$. \ben{To do}.
% 
% 		%%% Fourth Point
% 		\item \ben{[To generalize to shallow contexts]} By induction on $\evctx$. Cases:
% 		\begin{enumerate}
% 			\item \emph{Empty Context $\evctx = \ctxhole$}. By definition, $\unf\evctx\ctxholep{\relunf\tmtwo\evctx}$ is exactly $\unf\tm$.
% 			
% 			\item \emph{Application Left $\evctx = \evctxtwo\tmthree$}. Then 
% 			\[\begin{array}{lll}
% 				\unf\tm & =\\
%                                 \unf{(\evctxtwop\tmtwo\tmthree)} & =\\
%                                 \unf{\evctxtwop\tmtwo} \unf\tmthree & =_{\ih} \\
%                                 \unf\evctxtwo\ctxholep{\relunf\tmtwo\evctxtwo} \unf\tmthree & =\\
%                                 \unf{(\evctxtwo\tmthree)}\ctxholep{\relunf\tmtwo{\evctxtwo\tmthree}} & =\\
%                                 \unf\evctx\ctxholep{\relunf\tmtwo\evctx}
% 			\end{array}\]
% 			
% 			\item \emph{Application Right $\evctx = \tmthree\evctxtwo$}. Then 
% 			\[\begin{array}{lll}
% 				\unf\tm & =\\
%                                 \unf{(\tmthree\evctxtwop\tmtwo)} & =\\
%                                 \unf\tmthree \unf{\evctxtwop\tmtwo} & =_{\ih}\\
%                                 \unf\tmthree \unf\evctxtwo\ctxholep{\relunf\tmtwo\evctxtwo} & =\\
%                                 \unf{(\tmthree\evctxtwo)}\ctxholep{\relunf\tmtwo{\tmthree\evctxtwo}} & =\\
%                                 \unf\evctx\ctxholep{\relunf\tmtwo\evctx}
% 			\end{array}\]
% 
% 			\item \emph{Substitution $\evctx = \evctxtwo\esub\var\tmthree$}. Then 
% 			\[\begin{array}{lll}
% 				\unf\tm & =\\
%                                 \unf{\evctxtwop\tmtwo\esub\var\tmthree} 	 & =\\
%                                 \unf{\evctxtwop\tmtwo} \isub\var{\unf\tmthree} & =_{\ih}\\
%                                 \unf\evctxtwo\ctxholep{\relunf\tmtwo\evctxtwo}\isub\var{\unf\tmthree} & =_{\reflemmaeq{evctx-and-sub-commute}} \\
%                                 \unf\evctxtwo\isub\var{\unf\tmthree}\ctxholep{\relunf\tmtwo\evctxtwo\isub\var{\unf\tmthree}} & = \\
%                                 \unf{\evctxtwo\esub\var\tmthree}\ctxholep{\relunf\tmtwo{\evctxtwo\esub\var{\tmthree}}} & = \\\
%                                 \unf\evctx\ctxholep{\relunf\tmtwo\evctx}
% 			\end{array}\]
% 		\end{enumerate}
% 
% 	\end{enumerate}
\end{IEEEproof}
\end{atend}
%}


==> intro.tex <==
% !TEX root = main.tex
\section{Introduction}
The $\lambda$-calculus is an interesting computational model because it is machine-independent, simple to define, and it compactly models functional and higher-order logic programming languages. Its definition has only one rule, the $\beta$ rule, and no data structures. The catch is the fact that the $\beta$-rule---which by itself is Turing-complete---does not look as an atomic rule. Its action, namely $(\la\var\tm)\tmtwo \to_{\beta} \tm\isub\var\tmtwo$, can make many copies of an arbitrarily big sub-program $\tmtwo$. In other computational models like Turing or RAM machines, an atomic operation can be moving the head on the ribbon or accessing a register. Is $\beta$ atomic in that sense? Can one count the number of $\beta$-steps to the result and then claim that it is a reasonable bound on the complexity of the term? Intuition says no, because $\beta$ can be nasty, and make the program grow at an exponential rate. This is the \emph{size explosion problem}.

\paragraph*{Useful Sharing} nonetheless, it is possible to take the number of $\beta$-steps as an invariant cost model, \ie\ as a complexity measure polynomially related to RAM or Turing Machines. While this was known for some notable sub-calculi \cite{DBLP:conf/fpca/BlellochG95,DBLP:conf/birthday/SandsGM02,DBLP:journals/tcs/LagoM08,DBLP:journals/corr/abs-1208-0515,DBLP:conf/rta/AccattoliL12}, the first proof for the general case is a recent result by Accattoli and Dal Lago \cite{DBLP:conf/csl/AccattoliL14}. Similarly to the literature, they circumvent size explosion by factoring the problem via an intermediary model in between $\lambda$-calculus and machines. Their model is the \emph{linear substitution calculus} (LSC) \cite{DBLP:conf/popl/AccattoliBKL14,DBLP:conf/csl/AccattoliL14}, that is a simple $\lambda$-calculus with sharing annotations (also known as explicit substitutions) where the substitution process is decomposed in micro steps, replacing one occurrence at the time. In contrast with the literature, the general case is affected by a stronger form of size explosion, requiring an additional and sophisticated layer of sharing, called \emph{useful sharing}. Roughly, a micro substitution step is \emph{useful} if it contributes somehow to the creation of a $\beta$-redex, and \emph{useless} otherwise. Useful reduction then selects only useful substitution steps, avoiding the useless ones. In \cite{DBLP:conf/csl/AccattoliL14}, the Useful LSC is shown to be polynomially related to both $\l$-calculus (in a quadratic way) and RAM machines (with polynomial overhead, conjectured linear). It follows a polynomial relationship $\lambda \to \mbox{RAM}$. Pictorially:
\begin{center}
      \begin{tikzpicture}[ocenter]
       \node (l) {\small $\lambda$};
       \node at (l.center)  [right=2*\nodeHorDist](ram){\small RAM};
       \node at (l.center)  [right=\nodeHorDist](ghost) {};
       \node at (ghost.center)  [below =\nodeVerDist](ulsc) {\small Useful LSC};
       \draw[->, dotted] (l) to node {$polynomial$} (ram);
       \draw[->] (l) to node[below = 2pt, left =1pt] {$quadratic$} (ulsc);
       \draw[->] (ulsc) to node[below = 2pt, right =1pt, overlay] {{$polynomial\ \ (linear?)$}} (ram);
      \end{tikzpicture} 
\end{center}

Coming back to our questions, the answer of \cite{DBLP:conf/csl/AccattoliL14} is yes, $\beta$ is atomic, up to a polynomial overhead. It is natural to wonder how big is this overhead. Is $\beta$ reasonably atomic? Or the degree of the polynomial is big and the invariance result has only a theoretical value? In particular, in \cite{DBLP:conf/csl/AccattoliL14} the definition of useful steps relies on a \emph{separate} and \emph{global} test for usefulness, that despite being tractable might not be feasible in practice. Is there an efficient way to implement the Useful LSC? Does useful sharing---\ie\ the avoidance of useless duplications---bring a costly overhead? This paper answers these questions. But, in order to stress the practical value of the study, it shifts to a slightly different setting. 

\paragraph*{The Fireball Calculus} we recast the problem on the new \emph{fireball calculus} (\FC), essentially the weak call-by-value $\l$-calculus generalized to handle open terms. It is an intermediary step towards a strong call-by-value $\l$-calculus, that can be seen as iterated open weak evaluation. This approach to strong evaluation is followed also by Gregoire and Leroy in \cite{DBLP:conf/icfp/GregoireL02}. It avoids some of the complications of the strong case while its invariance already requires useful sharing, \ie\ it presents the same subtleties of the strong call-by-name case. 

Free variables are actually formalised using a distinguished syntactic class, that of \emph{\symbs}, noted $\const,\consttwo,\constthree$. This approach is technical convenient because allows to restrict to closed terms, so that any variable occurrence $\var$ is bound somewhere, while still having a representation of free variables (as \symbs).

The basic idea is that---in presence of \symbs---restricting $\beta$-redex to \emph{fire} only in presence of values is problematic. Consider indeed the following term:
$$\tm\defeq ((\la\var\la\vartwo\tmtwo)(\const\const))\tmthree$$
where $\tmthree$ is normal. For the usual call-by-value operational semantics $\tm$ is normal (because $\const\const$ is not a value) while for theoretical reasons (see \cite{DBLP:journals/ita/PaoliniR99,DBLP:conf/flops/AccattoliP12,DBLP:conf/fossacs/CarraroG14}) one would like to be able to fire the blocked redex, reducing to $(\la\vartwo\tmtwo\isub\var{\const\const})\tmthree$, so that a new redex is created and the computation can continue. According to the standard classification of redex creations due to \levy \cite{thesislevy}, this is a creation of type 1, and creations are a key concept in the study of invariance and usefulness.

The solution we propose here is to relax the constraint about values, allowing $\beta$-redexes to fire whenever the argument is a more general structure, called \emph{fireball} and defined recursively by extending values with \emph{inerts}, \ie\ applications of \symbs to fireballs. In particular, $\const\const$ is inert, so that \eg $\tm \to (\la\vartwo\tmtwo\isub\var{\const\const})\tmthree$, as desired.

Functional programming languages are usually modeled by weak and \emph{closed} calculi, so it is natural to wonder about the practical relevance of the \FC. Applications are along two axes. On the one hand, the evaluation mechanism at work in proof assistants has to deal with open terms for comparison and unification. For instance, Gregoire and Leroy's \cite{DBLP:conf/icfp/GregoireL02}, meant to improve the implementation of Coq, relies on the concept of inert (therein called \emph{accumulator}). On the other hand, \symbs may also be interpreted as special \emph{constructors} without destructors, meant to represent data as lists or trees. The dynamics of fireballs is in fact consistent with the way constructors are handled by Standard ML~\cite{citeulike:113339} and in several formalizations of core ML, as in~\cite{Clement:1986:SAL:319838.319847}. Therefore firing redexes involving inerts is also justified from a practical perspective. 

\paragraph*{The Relative Usefulness of Fireballs} as we explained, the generalization of values to fireballs is motivated by creations of type 1 induced by the firing of inerts. There is a subtlety, however. While \emph{substituting} a value can create a new redex (\eg\ as in $(\la\var(\var I)) I \to (\var I) \isub\var I = II$, where $I$ is the identity---these are called creations of type 3\footnote{\levy identifies 3 types of creations for the call-by-name $\l$-calculus. We mentioned types 1 and 3. The second case and the further cases specific to call-by-value are irrelevant for our study.}), substituting a inert can not. Said differently, duplicating inerts is useless, and leads to a strong form of size explosion, exactly as in the ordinary $\lambda$-calculus. Note the tension between different needs: redexes involving inerts have to be fired (for creations of type 1), and yet the duplication and the subtitution of inerts should be avoided (since they do not give rise to creations of type 3). We solve the tension by turning to useful sharing. Both values and inerts (\ie\ fireballs) will be shared, but only the substitution of values might be useful, because inerts are always useless. This is what we call \emph{the relative usefulness of fireballs}. It is also why---in contrast to Gregoire and Leroy---we do not identify fireballs and values.

\paragraph*{The Result} our main result is an implementation of \FC\ relying on useful sharing and such that---surprisingly---has only a linear overhead with respect to the number of $\beta$-steps. To be precise, the overhead is \emph{bilinear}, \ie\ linear in the number of $\beta$-steps \emph{and} in the size of the initial term (roughly the size of the input). The dependency from the size of the initial term is induced by the action of $\beta$ on whole subterms, rather than on atomic pieces of data as in Turing or random access machines. Therefore, $\beta$ is not exactly as atomic as accessing a register or moving the head of a turing machine, and this is the price to pay for embracing higher-order computations. Bilinearity, however, guarantees that such a price is mild and that the number of $\beta$ step---\ie\ of function calls in a functional program---is a faithful measure of the complexity of a program. To sum up, our answer is yes, $\beta$ is also reasonably atomic.

\paragraph*{A Receipt for Bilinearity, with Three Ingredients} our proof technique is a tour de force progressively combining together and adapting to the \FC\ three recent works involving the LSC, namely the already cited invariance of useful sharing of \cite{DBLP:conf/csl/AccattoliL14}, the tight relationship with abstract machines developed by Accattoli, Barenbaum, and Mazza in \cite{DBLP:conf/icfp/AccattoliBM14}, and the optimization of the substitution process studied by the present authors in \cite{DBLP:conf/wollic/AccattoliC14}. The next section will give an overview of these works and of how they are here combined, stressing how the proof is more than a simple stratification of techniques. In particular, it was far from evident that the orthogonal solutions introduced by these works could be succesfully combined together.


\paragraph*{This Paper} the paper is meant to be self-contained, and mostly follows a didactic style. For the first half we warm up discussing  design choices, the difficulty of the problem, and the abstract architecture. The second half focuses on the results. We also suggest to read the introductions of \cite{DBLP:conf/csl/AccattoliL14,DBLP:conf/icfp/AccattoliBM14,DBLP:conf/wollic/AccattoliC14}, because they provide intuitions about concepts that here are only hinted at. Although not essential, they will certainly soften the reading of this dense work. Omitted proofs are in the appendix and related work is discussed in \refsect{related-work}.

\section{A Receipt with Three Ingredients}
This section gives a sketch of how the bilinear implementation is built by mixing together tools from three different studies on the LSC.

\paragraph*{1) Useful Fireballs} we start by introducing the Useful Fireball Calculus (Useful \FC), akin to the Useful LSC, and provide the proof that the relationship \FC\ $\to$ \UsFC, analogously to the arrow $\l$ $\to$ Useful LSC, has a quadratic overhead. Essentially, this step provides us with the following diagram:
\begin{center}
      \begin{tikzpicture}[ocenter]
       \node (l) {\small $\FC$};
       \node at (l.center)  [right=2*\nodeHorDist](ram){\small RAM};
       \node at (l.center)  [right=\nodeHorDist](ghost) {};
       \node at (ghost.center)  [below =\nodeVerDist](ulsc) {\small Useful \FC};
       \draw[->, dotted] (l) to node {$polynomial$} (ram);
       \draw[->] (l) to node[below = 2pt, left =1pt] {$quadratic$} (ulsc);
       \draw[->] (ulsc) to node[below = 2pt, right =1pt] {$polynomial$} (ram);
      \end{tikzpicture} 
\end{center}
We go beyond simply adapting the study of \cite{DBLP:conf/csl/AccattoliL14}, as the use of evaluation contexts (typical of call-by-value scenarios) leads to the new notion of \emph{useful evaluation context}, that simplifies the technical study of useful sharing. Another key point is the \emph{relative usefulness of fireballs}, according to their nature: only values are properly subject to the useful discipline, \ie\ are duplicated only when they contribute somehow to $\beta$-redexes, while inerts are never duplicated.

\paragraph*{2) Distilling Useful Fireballs} actually, we do not follow \cite{DBLP:conf/csl/AccattoliL14} for the study of the arrow \UsFC\ $\to$ RAM. We rather refine the whole picture, by introducing a further intermediary model, an \emph{abstract machine}, mediating between the Useful \FC\ and RAM. We adopt the \emph{distillation technique} of \cite{DBLP:conf/icfp/AccattoliBM14}, that establishes a fine and modular view of abstract machines as strategies in the LSC up to a notion of structural equivalence on terms. The general pattern arising from \cite{DBLP:conf/icfp/AccattoliBM14} is that for call-by-name/value/need weak and closed calculi the abstract machine adds only a bilinear overhead with respect to the shared evaluation within the LSC: 
\begin{center}
      \begin{tikzpicture}[ocenter]
       \node (fc) {\small $\l$-Calculus};
       \node at (fc.center)  [right=2*\nodeHorDist](ram){\small RAM};
       \node at (fc.center)  [below =\nodeVerDist](ufc) {\small LSC};
       \node at (ram.center)  [below =\nodeVerDist](glam) {\small Abstract Machine};
       %\draw[->, dotted] (fc) to node {$quadratic$} (ram);
       \draw[->] (ufc) to node {$bilinear$} (glam);
       \draw[->] (fc) to (ufc);
       \draw[->] (glam) to node[right] {$bilinear$} (ram);
      \end{tikzpicture} 
\end{center}
Such \emph{distilleries} owe their name to the fact that the LSC retains only part of the dynamics of a machine. Roughly, it isolates the relevant part of the computation, distilling it away from the search of the next redex implemented by abstract machines. The search of the redex is mapped to a notion of  structural equivalence, a peculiar trait of the LSC, whose key property is that it can be postponed. Additionally, the transitions implementing the search of the next redex are proved to be bilinear in those simulated by the LSC: the LSC then turns out to be a complexity-preserving abstraction of abstract machines.


The second ingredient for the receipt is then a new abstract machine, called \glamour\ (for a reason), that we prove to implement the Useful \FC\ within a bilinear overhead. Moreover, the \glamour\ itself can be implemented within a bilinear overhead. Therefore, we obtain the following diagram:
\begin{center}
      \begin{tikzpicture}[ocenter]
       \node (fc) {\small \FC};
       \node at (fc.center)  [right=2*\nodeHorDist](ram){\small RAM};
       \node at (fc.center)  [below =\nodeVerDist](ufc) {\small Useful \FC};
       \node at (ram.center)  [below =\nodeVerDist](glam) {\small \glamour\ AM};
       \draw[->, dotted] (fc) to node {$quadratic$} (ram);
       \draw[->] (ufc) to node {$bilinear$} (glam);
       \draw[->] (fc) to node[left] {$quadratic$} (ufc);
       \draw[->] (glam) to node[right] {$bilinear$} (ram);
      \end{tikzpicture} 
\end{center}
This is the most interesting and original step of our study. First, it shows that distilleries are compatible with open terms and useful sharing. Second, while in \cite{DBLP:conf/icfp/AccattoliBM14} distilleries were mainly used to revisit machines in the literature, here the distillation principles are used to guide the design of a new abstract machine. Third, useful sharing is handled via a refinement of an ordinary abstract machine relying on a basic form of labelling. The most surprising fact is that such a labelling (together with invariants induced by the call-by-value scenario) allows a straightforward and very efficient implementation of useful sharing. While the calculus is based on \emph{separate} and \emph{global} tests for the usefulness of a substitution step, the labeling allows the machine to do \emph{on-the-fly} and \emph{local} tests, requiring only constant time (!). It then turns out that implementing usefulness is much easier than analizyng it. Summing up, useful sharing is easy to implement and thus a remarkable case of a theoretically born concept with relevant practical downfalls.

\paragraph*{3) Unchaining Substitutions}
at this point, it is natural to wonder if the bottleneck given by the side of the diagram \FC\ $\to$ \UsFC, due to the overhead of the decomposition of substitutions, can be removed. The bound on the overhead is in fact tight, and yet the answer is yes, if one refines the actors of the play. Our previous work \cite{DBLP:conf/wollic/AccattoliC14}, showed that (in ordinary weak and closed settings) the quadratic overhead is due to malicious chains of \emph{renamings}, \ie\ of substitutions of variables for variables, and that the substitution overhead reduces to linear if the evaluation is modified so that variables are never substituted, \ie\ if values do not include variables.

For the fireball calculus the question is tricky. First of all a disclaimer: with \emph{variables} we refer to occurrences of bound variables and not to \symbs/free variables. Now, our initial definition of the calculus will exclude variables from fireballs, but useful sharing will force to somehow reintroduce them. Our way out is an optimized form of substitution that \emph{unchains} renaming chains, and whose overhead is proved linear by a simple amortized analysis. Such a third ingredient is first mixed with both the \UsFC\ and the \glamour, obtaining the \FFC\ and the \Fglamour, and then used to prove our main result, an implementation \FC\ $\to$ RAM having an overhead linear in the number of $\beta$ steps and in the size of the initial term: 

\begin{center}
      \begin{tikzpicture}[ocenter]
       \node (fc) {\small \FC};
       \node at (fc.center)  [right=2*\nodeHorDist](ram){\small RAM};
       \node at (fc.center)  [below =\nodeVerDist](ufc) {\small \FFC};
       \node at (ram.center)  [below =\nodeVerDist](glam) {\small \Fglamour};
       \draw[->, dotted] (fc) to node {$bilinear$} (ram);
       \draw[->] (ufc) to node {$bilinear$} (glam);
       \draw[->] (fc) to node[left] {$linear$} (ufc);
       \draw[->] (glam) to node[right] {$bilinear$} (ram);
      \end{tikzpicture} 
\end{center}
In this step, the original content is that the unchaining obtimization---while inspired by \cite{DBLP:conf/wollic/AccattoliC14}---is subtler to define than in \cite{DBLP:conf/wollic/AccattoliC14}, as bound variables cannot be simply removed from the definition of fireballs, because of usefulness. Moreover, we also show how such an optimization can be implemented at the machine level.\medskip

The next section discusses related work. Then there will be a long preliminary part providing basic definitions, an abstract decomposition of the implementation, and a quick study of both a calculus, the \ShFC, and a machine, the \GLAM, without useful sharing. Both the calculus and the machine will not have any good asymptotical property, but they will be simple enough to familiarize with the framework and with the many involved notions.


\section{Related Work}
\label{sect:related-work}
In the literature invariance results for the weak
call-by-value $\l$-calculus have been proved three times,
independently. First, by Blelloch and Greiner
\cite{DBLP:conf/fpca/BlellochG95}, while studying cost models for
parallel evaluation. Then by Sands, Gustavsson and Moran
\cite{DBLP:conf/birthday/SandsGM02}, while studying speedups for
functional languages, and finally by Dal Lago and Martini
\cite{DBLP:journals/tcs/LagoM08}, who addressed the invariance thesis
for $\l$-calculus. Among them, \cite{DBLP:conf/birthday/SandsGM02} is the closest one, as it also provides an abstract machine and bounds its overhead. These works however concerns closed terms, and so they deal with a much simpler case. Other simple call-by-name cases are studied in \cite{DBLP:journals/corr/abs-1208-0515} and \cite{DBLP:conf/rta/AccattoliL12}. The difficult case of the strong $\l$-calculus has been studied in \cite{DBLP:conf/csl/AccattoliL14}, that is also the only reference for useful sharing. 

The LSC is a variation over a $\l$-calculus with ES by Robin Milner \cite{DBLP:journals/entcs/Milner07,KesnerOConchuir}, obtained by plugging in some of the ideas of the structural $\l$-calculus by Accattoli and Kesner \cite{DBLP:conf/csl/AccattoliK10}, introduced  as a syntactic reformulation of linear
logic proof nets. The LSC is similar to calculi studied by De Bruijn~\cite{deBruijn87} and Nederpelt~\cite{Ned92}. Its first appearances in the literature are in \cite{DBLP:conf/rta/AccattoliL12,DBLP:conf/rta/Accattoli12}, but its inception is actually due to Accattoli and Kesner.

Many abstract machines can be rephrased as strategies in \emph{$\l$-calculi with explicit substitutions} (ES), see at least \cite{DBLP:journals/tcs/Curien91,DBLP:journals/jfp/HardinM98,DBLP:journals/tocl/BiernackaD07,DBLP:journals/lisp/Lang07,DBLP:journals/lisp/Cregut07,DBLP:journals/toplas/AriolaBS09}.

The related work that is by far closer to ours is the already cited study by Gr\'egoire and Leroy of an abstract machine for call-by-value weak and open reduction in \cite{DBLP:conf/icfp/GregoireL02}. We developed our setting independently, and yet the \FC\ is remarkably close to their calculus, in particular our \emph{fireballs} are essentially their \emph{accumulators}. The difference is that our work is complexity-oriented while theirs is implementation-oriented. On the one hand they do not recognize the relative usefulness of fireballs, and so their machine is not invariant, \ie\ our machine is more efficient and on some terms even exponentially faster. On the other hand, they extend the language up to the calculus of constructions, present a compilation to bytecode, and certify in Coq the correctness of the implementation.

The abstract machines in this paper use \emph{global} environments, an approach followed only by a minority of authors  
\cite{DBLP:conf/birthday/SandsGM02,DBLP:journals/entcs/FernandezS09,DBLP:conf/ppdp/DanvyZ13,DBLP:conf/icfp/AccattoliBM14} and essentially identifying the environment with a store.

The distillation technique was developed to better understand the relationship between the KAM and weak linear head reduction pointed out by Danos \& Regnier \cite{Danos04headlinear}. The idea to distinguish between \emph{operational content} and \emph{search of the redex} in an abstract machine is not new, as it underlies in particular the \emph{refocusing semantics} of Danvy and Nielsen \cite{Danvy04refocusingin}. Distilleries bring however an original refinement where logic, rewriting, and complexity color the picture, leading to formal bounds on machine overheads.

Our unchaining optimization is a lazy variant of an optimization repeatedly appeared in the literature on abstract machines, often with reference to space consumption and \emph{space leaks}, for instance in \cite{DBLP:conf/birthday/SandsGM02} as well as in Wand's \cite{DBLP:journals/lisp/Wand07} (section 2), Friedman et al.'s \cite{DBLP:journals/lisp/FriedmanGSW07} (section 4), and Sestoft's \cite{DBLP:journals/jfp/Sestoft97} (section 4).


==> macros/moveproofs.tex <==
\usepackage{etex,etoolbox}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{environ}

\makeatletter
\providecommand{\@fourthoffour}[4]{#4}
% We define an addition for the theorem-like environments; when
% \newtheorem{thm}{Theorem} is declared, the macro \thm expands
% to {...}{...}{...}{Theorem} and with \@fourthoffour we access
% to it; then we make available \@currentlabel (the theorem number)
% also outside the environment.  
\newcommand\fixstatement[2][\proofname\space of]{%
  \ifcsname thmt@original@#2\endcsname
    % the theorem has been declared with \declaretheorem
    \AtEndEnvironment{#2}{%
      \xdef\pat@label{\expandafter\expandafter\expandafter
        \@fourthoffour\csname thmt@original@#2\endcsname\space\@currentlabel\space(page \thepage)}%
      \xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
    }%
  \else
    % the theorem has been declared with \newtheorem
    \AtEndEnvironment{#2}{%
      \xdef\pat@label{\expandafter\expandafter\expandafter
        \@fourthoffour\csname #1\endcsname\space\@currentlabel\thepage}%
      \xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
    }%
  \fi
  \@namedef{pat@proofof@#2}{#1}%
}

% We allocate a block of 1000 token registers; in this way \prooftoks
% is 1000 and we can access the following registers of the block by
% \prooftoks+n (0<n<1000); we'll use a dedicated counter for it
% that is stepped at every proof
\globtoksblk\prooftoks{1000}
\newcounter{proofcount}

% We gather the contents of the proof as argument to \proofatend
% and then we store
% "\begin{proof}[Proof of <theoremname> <theoremnumber>]#1\end{proof}"
% in the next token register of the allocated block
\NewEnviron{proofatend}{%
  \edef\next{%
    \noexpand{\unexpanded\expandafter{~\\\noindent \bf} Proof of \pat@label}
    \noexpand\begin{IEEEproof}%[\pat@proofof\space\pat@label]%
    \unexpanded\expandafter{\BODY}}%
  \global\toks\numexpr\prooftoks+\value{proofcount}\relax=\expandafter{\next\end{IEEEproof}~}
  \stepcounter{proofcount}}

\NewEnviron{atend}{%
  \edef\next{%
    \noexpand~%
    \unexpanded\expandafter{\BODY}}%
  \global\toks\numexpr\prooftoks+\value{proofcount}\relax=\expandafter{\next~}
  \stepcounter{proofcount}}

% \printproofs simply loops over the used token registers of the
% block, freeing their contents
\def\printproofs{%
  \count@=\z@
  \loop
    \the\toks\numexpr\prooftoks+\count@\relax
    \ifnum\count@<\value{proofcount}%
    \advance\count@\@ne
  \repeat}
\makeatother

%\declaretheorem[style=plain,name=Theorem,qed=$\square$,numberwithin=section]{thm}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma} \fixstatement{lemma}
\newtheorem{corollary}{Corollary} \fixstatement{corollary}
\newtheorem{theorem}{Theorem} \fixstatement{theorem}
\newtheorem{proposition}{Proposition} \fixstatement{proposition}
\newtheorem{remark}{Remark} \fixstatement{remark}


%\begin{document}
%\begin{lem}\label{addition}
%$1+1=2$
%\end{lem}
%\begin{proofatend}
%It's quite clear.
%\end{proofatend}

%\begin{thm}
%$1+2=3$
%\end{thm}
%\begin{proofatend}
%Obvious from lemma \ref{addition}.
%\end{proofatend}


==> pre-useful-machine.tex <==
% !TEX root = main.tex
\subsection{The GLAMoUr Machine}\label{sect:glamour}
\begin{atend}\subsection{Proofs Omitted From \refsect{glamour}\\ (The GLAMoUr Machine)}\end{atend}
\begin{atend}
The aim of this section is to prove \refth{uglam-refl-distillation}
($(\glamour,\togenu, \eqstruct, \decodefun)$ is a reflective explicit distillery) and \refth{preusefulimpl}
(the useful implementation has bilinear low level and quadratic high level
complexity). We start by proving that the invariants of the machine holds.

\end{atend}
Here we refine the GLAM with a very simple tagging of stacks and environments, in order to implement useful sharing. The idea is that every term in the stack or in the environment carries a label $\lab\in\set{\alive,\dead}$ indicating if it unfolds (relatively to the environment) to an abstraction or to a generalized constant. Then, terms marked $\alive$ when the context is empty and
terms marked $\dead$ are never duplicated.

The grammars are identical to the GLAM, up to labels:
$$\begin{array}{rclllrcllllllll}
        \lab & \grameq & \alive \mid \dead &&&&
%        \stackitem & \grameq & \code \mid \pair{\code}{\stack}\\
	\genv,\genvtwo		& \grameq & \stempty \mid  \econsx{\esub\var{\stackitem^\lab}}{\genv}\\
	\stack,\stacktwo 	& \grameq & \stempty \mid \stackitem^\lab \cons \stack
	%\dump, \dumptwo	& \grameq & \stempty \mid \dump \cons \nfnst\code\stack \\
\end{array}$$

The decoding of the various machine components is identical to that for the
GLAM, up to labels that are ignored. The state context, however, now is noted $\tctx_\state$, as it is not necessary an evaluation context. The transitions, given in \reftab{pre-useful-transitions}, are obtained from those
of the GLAM by 1) duplicating the commutative rules for constants and
abstractions so that a variable $\var$ is handled as a constant if bound
in the environment with label $\dead$, and as a value if bound in the
environment with label $\alive$; 2) restricting the exponential rule to expand
only variables bound with label $\alive$.


%The decoding of the various components is defined by:
%\begin{center}
%$\begin{array}{rclllllllllll}
	%\decode{\stempty}								& \defeq & \ctxhole \\
        %\decode{\pair{\tm}{\stack}} & \defeq & \decstackp{\tm} \\
	%\decode{ \stackitem^\lab \cons \stack} 				& \defeq & \decstackp{\ctxhole\decode{\stackitem}} \\
	%\decode{\dump\cons\dentry\tm\stack} 	& \defeq & \decdumpp{\decstackp{\tm \ctxhole}}\\
        %\decode{\genv\cons\esub\var{\stackitem^\lab}} & \defeq & \decgenvp{\ctxhole\esub\var{\decode\stackitem}}\\
        %\decode{\usefmac\genv\dump\code\stack)} & \defeq & \decgenvpx{\genv}{\decdumpp{\decstackp{\code}}}\\
%\end{array}$
%\end{center}

\begin{atend}
\begin{lemma}[Contextual Decoding]\label{l:contextualdecoding}
$\decgenv$ is a substitution context; $\decdump$ and $\decstack$ are
shallow contexts without ES.
\end{lemma}
\begin{IEEEproof}
by induction on $\genv$, $\dump$ and $\stack$.
\end{IEEEproof}
\end{atend}

%\begin{definition}[Well Named State]
%A state is \emph{well named} when all bound variables are pairwise distinct.
%\end{definition}

%Well namedness is required for the determinism of the machine and lack of
%crashes. For the determinism, the important part is that all variables bound
%in the environment should be pairwise distinct. The stronger requirement is
%to preserve well namedness as an invariant during computation.

\begin{lemma}[GLAMoUr Invariants]\label{l:uglaminvariants} % \reflemmap{uglaminvariants}{value}
	Let $\state = \usefmac{\genv}{\dump}{\codetwo}{\stack} $ be a state reachable from an initial code $\code$. Then:
	\begin{enumerate}
		\item \emph{Closure}:\label{p:uglaminvariants-closure} $\state$ is closed and well named;
		\item \emph{Value}:\label{p:uglaminvariants-value} values in components of $\state$ are sub-terms of $\code$;
		\item \emph{\Fireball}:\label{p:uglaminvariants-fireball} $\relunf\code{\decgenv}$ is a fireball (of kind $\lab$) for every code $\code^\lab$ in $\stack$, $\genv$, and in every stack of $\dump$;
		\item \emph{Evaluability}:\label{p:uglaminvariants-eval} $\decode\genv$, $\relunf{\decdump}{\decode\genv}$, $\relunf{\decstack}{\decode\genv}$, and $\tctx_\state$ are evaluable contexts;
		\item \emph{Environment Size}:\label{p:uglaminvariants-size} the length of the global environment $\genv$ is
bound by $\sizem\exec$.
	\end{enumerate}
\end{lemma}

\begin{proofatend}
by induction over the length of the execution.
The base case holds because $\code$ is initial.
The inductive step is by cases over the kind of transition.
All the verifications are trivial apart for \refpoint{uglaminvariants-eval}. For \refpoint{uglaminvariants-eval}, evaluability for $\decode\genv$, $\relunf{\decdump}{\decode\genv}$, $\relunf{\decstack}{\decode\genv}$ follows from \refpoint{uglaminvariants-fireball} and \reflemmap{evaluable-prop}{five}, while evaluability for $\decgenvpx{\genv}{\decdumpp{\decstack}}$ follows from them and \reflemmap{evaluable-prop}{five}.
\end{proofatend}

\begin{atend}

\begin{lemma}[Explicit Distillation]\label{l:uglam-distillation}
	Let $\state$ be a reachable state. Then:
		\begin{enumerate}
		\item \emph{Commutative}: if $\state\tomachcp{_{1,2,3,4,5}}\statetwo$ then $\decode\state = \decode\statetwo$;
		\item \emph{Multiplicative}: if $\state\tomachum\statetwo$ then $\decode\state\togenum\eqstruct\decode\statetwo$;
		\item \emph{Exponential}: if $\state\tomachue\statetwo$ then $\decode\state\togenue\decode\statetwo$.
	\end{enumerate}
\end{lemma}

\begin{IEEEproof}
we list the transition in the order they appear in the definition of the machine.
\begin{itemize}
\item
Case
     $\usefmac{\genv}{\dump}{\code\codetwo}{\stack}
     \tomachcone
     \usefmac{\genv}{\dump\cons\nfnst\code\stack}{\codetwo}{\stempty}$:
 $$\begin{array}{ll}
     \decode{\usefmac{\genv}{\dump}{\code\codetwo}{\stack}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\codetwo}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\ctxholep{\codetwo}}{\stack}}} 
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\codetwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\codetwo}{\stempty}}}
     &=\\
     \decode{\usefmac{\genv}{\dump\cons\nfnst\code\stack}{\codetwo}{\stempty}}
 \end{array}$$

\item
Case 
     $\usefmac{\genv}{\dump}{\l\var.\code}{\stackitem^\lab\cons\stack}
     \tomachum
     \usefmac{\esub\var{\stackitem^\lab}\genv}{\dump}{\code}{\stack}$:
 $$\begin{array}{lll}
     \decode{\usefmac{\genv}{\dump}{\l\var.\code}{\stackitem^\lab\cons\stack}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\l\var.\code}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{(\l\var.\code)\decode{\stackitem}}{\stack}}}
     &\togenum&\mbox{(by \reflemmap{uglaminvariants}{eval}}\\&&\mbox{and \reflemmap{uglaminvariants}{fireball})}\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\esub{\var}{\decode{\stackitem}}}{\stack}}}
     &\eqstruct&\mbox{(by \reflemma{ev-comm-struct})}\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{\stack}}\esub\var{\stackitem}}
     &=\\
     \decgenvpx{\esub\var{\stackitem^\lab}\genv}{\decodep{\dump}{\decodestack{\code}{\stack}}}
     &=\\
     \decode{\usefmac{\econs{\esub\var{\stackitem^\lab}}{\genv}}{\dump}{\code}{\stack}}
 \end{array}$$

\item
Case
     $\usefmac{\genv}{\dump\cons\nfnst\code\stack}{\const}{\stacktwo}
     \tomachctwo
     \usefmac{\genv}{\dump}{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}$:
 $$\begin{array}{ll}
     \decode{\usefmac{\genv}{\dump\cons\nfnst\code\stack}{\const}{\stacktwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\decode{\const}}{\stacktwo}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\decodestack{\const}{\stacktwo}}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}}}
     &=\\
     \decode{\usefmac{\genv}{\dump}{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}}
 \end{array}$$

\item
Case
     $\usefmac{\genv_1\esub\var{\stackitem^\dead}\genv_2}{\dump\cons\nfnst\code\stack}{\var}{\stacktwo}
     \tomachcthree
     \usefmac{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump}{\code}{\pair{\var}{\stacktwo}^\dead\cons\stack}$:
 $$\begin{array}{ll}
     \decode{\usefmac{\genv_1\esub\var{\stackitem^\dead}\genv_2}{\dump\cons\nfnst\code\stack}{\var}{\stacktwo}}
     &=\\
     \ldots&=\\
     \decode{\usefmac{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump}{\code}{\pair{\var}{\stacktwo}^\dead\cons\stack}}
 \end{array}$$
The proof is the one for the previous case $\tomachctwo$,
by replacing $\const$ with $\var$ and instantiating $\genv$ with
${\genv_1\esub\var{\phi^\dead}\genv_2}$.

\item
Case
     $\usefmac{\genv}{\dump\cons\nfnst\code\stack}{\l\var.\codetwo}{\stempty}
     \tomachcfour
     \usefmac{\genv}{\dump}{\code}{(\l\var.\codetwo)^\alive\cons\stack}:$
 $$\begin{array}{ll}
     \decode{\usefmac{\genv}{\dump\cons\nfnst\code\stack}{\l\var.\codetwo}{\stempty}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\l\var.\codetwo}{\stempty}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\l\var.\codetwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code(\l\var.\codetwo)}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{(\l\var.\codetwo)^\alive\cons\stack}}}
     &=\\
     \decode{\usefmac{\genv}{\dump}{\code}{(\l\var.\codetwo)^\alive\cons\stack}}
 \end{array}$$

\item
Case
     $\usefmac{\genv_1\esub\var{\codetwo^\alive}\genv_2}{\dump\cons\nfnst\code\stack}{\var}{\stempty}
     \tomachcfive
     \usefmac{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump}{\code}{\var^\alive\cons\stack}$:
 $$\begin{array}{ll}
     \decode{\usefmac{\genv_1\esub\var{\codetwo^\alive}\genv_2}{\dump\cons\nfnst\code\stack}{\var}{\stempty}}
     &=\\
     \ldots&=\\
     \decode{\usefmac{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump}{\code}{\var^\alive\cons\stack}}
 \end{array}$$
The proof is the one for the previous case $\tomachcfour$,
by replacing $(\l\var.\codetwo)$ with $\var$ and instantiating
$\genv$ with ${\genv_1\esub\var{\herval{\codetwo}}\genv_2}$.

\item
Case
     $\usefmac{\genv_1\esub\var{\herval\codevalt}\genv_2}{\dump}{\var}{\stackitem^\lab\cons\stack}
     \tomachee
     \usefmac{\genv_1\esub\var{\herval\codevalt}\genv_2}{\dump}{\rename\codevalt}{\stackitem^\lab\cons\stack}$:
 $$\begin{array}{lll}
     \decode{\usefmac{\genv_1\esub\var{\herval\codevalt}\genv_2}{\dump}{\var}{\stackitem^\lab\cons\stack}}
     &=\\
     \decgenvpx{\genv_1\esub\var{\herval\codevalt}\genv_2}{\decodep{\dump}{\decodestack{\var}{\stackitem^\val\cons\stack}}}
     &\togenue&\mbox{(by \reflemmap{uglaminvariants}{eval}}\\&&\mbox{and \reflemmap{uglaminvariants}{fireball})}\\
     \decgenvpx{\genv_1\esub\var{\herval\codevalt}\genv_2}{\decodep{\dump}{\decodestack{\rename\codevalt}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decode{\usefmac{\genv_1\esub\var{\herval\codevalt}\genv_2}{\dump}{\rename\codevalt}{\stackitem^\lab\cons\stack}}
 \end{array}$$
\end{itemize}
\end{IEEEproof}


The next lemma extends the notion of state size $\size\state$ given in
\refdef{sizetwo} by ignoring the new machine component $\genv$.
The precise definition is \refdef{presize}.

\begin{lemma}[Determinism]\label{l:uglam-deterministic} The reduction relation $\tomach$ is deterministic.
\end{lemma}
\begin{IEEEproof}
a simple inspection of the reduction rules shows no critical pairs.
\end{IEEEproof}

\begin{lemma}[Progress]\label{l:preprogress}
if $\state$ is reachable, $\admnf{\state}=\state$ and $\decode\state\togenx\tm$ with $\mathtt{x}\in\set{\usym\msym,\usym\esym}$, then there exists $\statetwo$  such that $\state\tomachx\statetwo$, \ie, $\state$ is not final.
\end{lemma}
\begin{IEEEproof}
by \reflemma{uglam-deterministic} and \reflemma{uglam-distillation} it is sufficient to show that every reachable stuck state decodes to a normal form. The only stuck forms are:
\begin{itemize}
 \item \emph{Error states}. The state con only be $\usefmac{\genv}{\dump}{\var}{\stack}$ where $\var$ is not defined
  in $\genv$ or it is defined to be a $\herval\code$ where $\code$ is not
  a variable or a value.\\
   The state is not reachable because it would violate either the
   invariant in \reflemmap{uglaminvariants}{closure} or the invariant in
   \reflemmap{uglaminvariants}{fireball}.

 \item \emph{Final states}. Cases:
 \begin{enumerate}
  \item \emph{The result is/unfolds to a value}. The state is $\usefmac{\genv}{\dumpempty}{\code}{\stempty}$
   with $\code$ an abstraction or a variable bound in
   $\genv$ to a $\stackitem^\alive$.
   By \reflemma{contextualdecoding},
   $\decode{\usefmac{\genv}{\dumpempty}{\code}{\stempty}} =
    \decgenvpx{\genv}{\code} = \sctxp\code$ for some $\sctx$.
   Note that $\unf{\sctxp\code} = \relunf\code\sctx$ is a \fireball, indeed if $\code$ is an abstraction it is given by \reflemma{es-answers-are-normal} and if it as a variable it is given by \reflemmap{uglaminvariants}{fireball}.
   Thus by \reflemma{useful-projection}, $\sctxp\code$ is normal.

  \item \emph{The result is/unfolds to a generalized constant}. The state is $\usefmac{\genv}{\dumpempty}{\code}{\stack}$
   with $\code$ a constant $\const$ or a variable bound in $\genv$ to a $\stackitem^\dead$.\\
   By \reflemma{contextualdecoding},
   $\decode{\usefmac{\genv}{\dumpempty}{\code}{\stack}} = \decgenvpx{\genv}{\decodestack{\code}{\stack}} = 
    \sctxp{\decodestack{\code}{\stack}}$ for some $\sctx$.
   Note that $\unf{\sctxp\code} = \relunf\code\sctx$ is a \fireball, indeed if $\code$ is a constant it is given by \reflemma{es-answers-are-normal} and if it as a variable it is given by \reflemmap{uglaminvariants}{fireball}.
   Moreover, by \reflemmap{uglaminvariants}{fireball},
   $\relunf{\decstack}\sctx$ has the form
   $\ctxhole\fire_1\ldots\fire_n$.
   Thus, by \reflemmap{relunf-properties}{zero} and the definition of fireballs,
   $\relunf{\decodestack{\code}{\stack}}{\sctx}$ is a fireball too.
   Therefore by \reflemma{useful-projection}, $\sctxp{\decodestack{\code}{\stack}}$ is normal.\qedhere
  \end{enumerate}
\end{itemize}
\end{IEEEproof}

\end{atend}

\begin{theorem}[\glamour\ Distillation]\label{th:uglam-refl-distillation}
	$(\glamour,\togenu, \eqstruct, \decodefun)$ is a reflective explicit distillery. In particular, let $\state$ be a reachable state:
	\begin{enumerate}
	  \item \emph{Commutative}: if $\state\tomachcp{_{1,2,3,4,5}}\statetwo$ then $\decode\state = \decode\statetwo$;
	  \item \emph{Multiplicative}: if $\state\tomachum\statetwo$ then $\decode\state\togenum\eqstruct\decode\statetwo$;
	  \item \emph{Exponential}: if $\state\tomachue\statetwo$ then $\decode\state\togenue\decode\statetwo$.
	\end{enumerate}
\end{theorem}

\begin{proofatend}
the theorem follows from \reflemma{uglam-distillation}, \reflemma{uglam-deterministic} and \reflemma{preprogress}.
\end{proofatend}
 
 In fact, the distillery is even bilinear, as we now show. The proof employs
 the following definition of size of a state.

\begin{definition}
  \label{def:presize}
  The \emph{size} of codes and states is defined by:
$$\begin{array}{rclllrclllll}
      \size{\var} = \size{\const}  	& \defeq & 1&&
      \size{\code\codetwo}		 	& \defeq & \size{\code} + \size{\codetwo}+1\\
      \size{\l \var.\code} 		& \defeq & \size{\code} + 1&&

      \size{\glam\genv\dump\code\stack} & \defeq & \size\code + \Sigma_{\nfnst\codetwo\stack \in \dump} \size\codetwo
  \end{array}$$
\end{definition}

\begin{lemma}[Size Bounded]
  \label{l:useful-dump-size-bounded}
 Let $\state=\usefmac\genv\dump\codetwo\stack$ be a state reached by an execution $\exec$ of initial code $\code$. Then
 $\size{\state} \leq (1+\sizeuee{\exec})\size{\code} - \sizecom{\exec}$.
\end{lemma}
\begin{IEEEproof}
by induction over the length of the derivation. The property trivially holds for the empty derivation. Case analysis over the
last machine transition. \emph{Commutative rule} $\tomachcone$: the rule splits the code $\code\codetwo$ between the dump and the code, and the measure---as well as the rhs of the formula---decreases by 1 because the rule consumes the application node. \emph{Commutative rules} $\tomachcp{_{2,3,4,5}}$: these rules consume the current code, so they decrease the measure of at least 1. \emph{Multiplicative}: it consumes the lambda abstraction.  \emph{Exponential}: it modifies the current code by replacing a variable (of size 1) with a value $\codeval$ coming from the environment. Because of \reflemmap{uglaminvariants}{value}, $\codeval$ is a sub-term of $\code$ and the dump size increment is bounded by $\size\code$.
\end{IEEEproof}

\begin{corollary}[Bi-linearity of $\tomachc$]
\label{coro:preuseful-bound1}
 Let $\state$ be a state reached by an execution $\exec$ of initial code $\code$. Then
 $\sizecom{\exec} \leq (1+\sizee{\exec})\size{\code} = O(\sizee{\exec}\cdot\size{\code})$.
\end{corollary}

Finally, we obtain our first implementation theorem.
\begin{table*}
\caption{Identity, Chain, and Chain-Starting Context + Rewriting Rules of the \FFC}
\label{tab:useful-rewritingrules}
\centering
\begin{tabular}{r|lccc}
\begin{tabular}{c}
$\begin{array}{lllllllllllll}
	\ictx, \ictxtwo			& \grameq & \ctxhole \mid \ictxp\var\esub\var\ictxtwo \mid \ictx\esub\var\tm\\
	\pevctx,\pevctxtwo 	& \grameq & \tctxp\var\esub{\var}{\ictx} \mid \pevctxp\var\esub{\var}{\ictx} \mid \tctxp\pevctx\\\\\cline{1-3}\\
	\end{array}$
	\\
	$\begin{array}{lllllllllllll}
		\tpctx{\tctxtwop\vartwo\esub{\vartwo}{\ictx}}{\var} & \defeq& \tctxtwo\esub{\vartwo}{\ictxp\var}\\
		\tpctx{\pevctxp\vartwo\esub{\vartwo}{\ictx}}{\var} & \defeq& \tpctx{\pevctx}{\vartwo}\esub{\vartwo}{\ictxp\var}\\
		\tpctx{\tctxtwop\pevctx}{\var} & \defeq& \tctxtwop{\tpctx{\pevctx}{\var}}
	\end{array}$
	\end{tabular}
	&
$\begin{array}{c@{\hspace{0.6cm}}l}
  \textsc{Rule (Already Closed by Contexts)} & \textsc{Side Condition} \\
	\tctxp{\sctxp{\l\var.\tm}\tmtwo} \togenlum \tctxp{\sctxp{\tm\esub\var\tmtwo}} &
	\mbox{$\tctxp{\ctxhole\tmtwo}$ is evaluable (and applicative)}\\\\
    
			\tctxp{\tctxtwop\var\esub\var{\sctxp{\valp}}} \togenluee  \tctxp{\sctxp{\tctxtwop\valp\esub\var\valp}} &
			    \mbox{$\tctxp{\tctxtwo\esub\var{\sctxp{\valp}}}$ is 
			     evaluable and applicative}\\\\


		\tctxp{\pevctxp\var\esub\var{\sctxp\valp}} \togenluei  \tctxp{\sctxp{\pevctxp\valp\esub\var\valp}} &
 	\mbox{$\tctxp{\tpctx\pevctx\var\esub\var{\sctxp\valp}}$ is
evaluable and applicative}
\end{array}$
\\
	

\end{tabular}
\end{table*}

\begin{theorem}[Useful Implementation]\label{th:preusefulimpl}\hfill
 \begin{enumerate}
  \item \emph{Low-Level Bilinear Implementation}: a $\togenu$-derivation $\deriv$ is implementable on RAM in $O(\size\tm\cdot \size\deriv)$ (\ie\ bilinear) steps.
  \item \emph{Low + High Quadratic Implementation}: a $\tof$-derivation $\deriv$ is implementable on RAM in $O(\size\tm\cdot \size\deriv^2)$ steps, \ie\ linear in the size of the initial term $\tm$ and quadratic in the length of the derivation $\size\deriv$.
 \end{enumerate}
 \end{theorem}

\begin{proofatend}
the proof follows from
\refthm{hlithm} applied to \refthm{quadratichlis},
and \refth{lowlevelimplth} applied to \refth{uglam-refl-distillation} and \refcoro{preuseful-bound1}.
Bi-linearity of the machine requires to show that the commutative steps are implementable in constant time, while the principal ones in time $O(\size\tm)$. The machine is meant to be implemented using a representation of codes using pointers, in particular for variables, so that the environment can be accessed in constant time. Assuming this, all rules except the exponential one evidently take constant time on a RAM machine, because they amount to moving pointers. The exponential rule requires $O(\size\tm)$ because it copies and $\alpha$-renames a value $\val$. Both these operations take time $O(\size\val)$. The value invariant (\reflemmap{uglaminvariants}{value}) guarantees $\size\val\leq\size\tm$. Additional considerations on the cost of similar rules can be found in \cite{DBLP:conf/icfp/AccattoliBM14} (page 9 and 11, paragraphs \emph{Abstract Considerations on Concrete Implementations}).
\end{proofatend}


==> pre-useful.tex <==




==> size-explosion.tex <==
% !TEX root = main.tex
\section{Size Explosion}
\label{sect:size-exp}
Size Explosion is the side effect of a discrepancy between the dynamics and the representation of terms. The usual substitution $\tm\isub\var\tmtwo$ makes copies of $\tmtwo$ for all the occurrences of $\var$, even if $\tmtwo$ is \emph{useless}, \ie\ it is normal and it does not create redexes after substitution. These copies are the burden leading to the exponential growth of the size. To illustrate the problem, let's build a size exploding family of terms. 

Note that a inert $\gconst$, when applied to itself still is a inert $\gconst\gconst$. In particular, it still is a fireball, and so it can be used as an argument for redexes. We can then easily build a term of size linear in $n$ that in $n$ steps evaluates a complete binary tree $\gconst^{2^n}$. Namely, define the family of terms $\tm_n$ for $n\geq1$:
\begin{center}$\begin{array}{lllllllll}
	\tm_1 & \defeq & \la{\var_{1}}(\var_{1}\var_{1})\\
	\tm_{n+1} & \defeq & \la{\var_{n+1}}(\tm_{n}(\var_{n+1}\var_{n+1}))
\end{array}$\end{center}

Now consider $\tm_n \gconst$, that for a fixed $\gconst$ has size linear in $n$. The next proposition shows that $\tm_n \gconst$ reduces in $n$ steps to $ \gconst^{2^n}$, causing size-explosion.

\begin{proposition}[Size Explosion in the \fb]
	$\tm_n \gconst \tof^n \gconst^{2^n}$.
\end{proposition}
\begin{IEEEproof}
	By induction on $n$. Let $\gconsttwo \defeq \gconst^2 = \gconst \gconst$. Cases:
$$\begin{array}{llllll}
	\tmtwo_1 & = & (\la{\var_{1}}(\var_{1}\var_{1})) \gconst &	\tof & \gconst^2	\\
	\tmtwo_{n+1} & = & (\la{\var_{n+1}}(\tm_{n}(\var_{n+1}\var_{n+1}))) \gconst & \tof \\
	& & \tm_n \gconst^2 = \tm_n \gconsttwo & \tof^n&&\mbox{(\ih)}\\
	& & \gconsttwo^{2^n} & = & \gconst^{2^{n+1}} & \hfill\qedhere
\end{array}$$
\end{IEEEproof}


==> useful-commutative-analysis.tex <==
% !TEX root = main.tex
%\subsection{Principal vs Commutative Analysis}

Bilinearity wrt $\tomachcp{_{1,2,3,4,5}}$ is identical to that of the \glamour, thus we omit it and focus on $\tomachcsix$.

\begin{atend}
~

In the remaining of the appendix we prove bilinearity of $\tomachcp{}$.
We begin redoing the proof for $\tomachcp{_{1,2,3,4,5}}$, that is almost
identical to that of the \glamour.

\begin{lemma}[Size Bounded]
 Let $\state=\usefmac\genv\dump\codetwo\stack$ be a state reached by an execution $\exec$ of initial code $\code$. Then
 $\size{\state} \leq (1+\sizeuee{\exec})\size{\code} - \sizecomphone{\exec}$.
\end{lemma}
\begin{IEEEproof}
the same reasoning as for the non-optimized case (\reflemma{useful-dump-size-bounded}) provides the proof for $\tomachm, \tomachee, \tomachcp{_{1,2,3,4,5}}$, while for the new transitions $\tomachcsix$ and $\tomachei$ it is enough to note that they do not change the size of the state.
\end{IEEEproof}

\begin{corollary}[Termination and Bilinearity of $\tomachcp{_{1,2,3,4,5}}$]
\label{coro:lazy-useful-bound1}
 Let $\state$ be a state reached by an execution $\exec$ of initial code $\code$. Then
 $\sizecomphone{\exec} \leq (1+\sizee{\exec})\size{\code} = O(\sizep{\exec}\cdot\size{\code})$. In particular, $\tomachcp{_{1,2,3,4,5}}$ terminates.
\end{corollary}

\end{atend}
The size $\size\heap$ of a chain heap is its length as a list.


\begin{lemma}[Linearity of $\tomachcsix$]
\label{l:heap-bound} % 
  Let $\state=\mac\genv\dump\heap\code\stack$ be a state reached by an execution $\exec$. Then 
  \begin{enumerate}
   \item \label{p:heap-bound-comm} $\sizecomsix\exec = \size\heap + \sizeuei\exec$.
   \item \label{p:heap-bound-heap} $\size\heap \leq \sizem\exec$.
   \item \label{p:heap-bound-final} $\sizecomsix\exec \leq \sizem\exec + \sizeuei\exec = O(\sizep{\exec})$.
  \end{enumerate}

\end{lemma}
\begin{IEEEproof}
\emph{1)} By induction over $\size\exec$ and analysis of the
last machine transition.
The $\tomachcsix$ steps increment the size of the heap. The $\tomachei$ steps
decrement it. All other steps do not change the heap. \emph{2)} By the compatible heap invariant (\reflemmap{lazy-uglaminvariants}{heap}), $\size\heap \leq \size\genv$. By the environment size invariant (\reflemmap{lazy-uglaminvariants}{size}), $\size\genv \leq \sizem\exec$. Then $\size\heap \leq \sizem\exec$. \emph{3)}  Plugging \refpoint{heap-bound-heap} into \refpoint{heap-bound-comm}.
\end{IEEEproof}


\begin{corollary}[Bilinearity of $\tomachc$]
\label{coro:useful-bound1}
 Let $\state$ be a state reached by an execution $\exec$ of initial code $\code$. Then
 $\sizecom{\exec} \leq (1+\sizee{\exec})\size{\code} + \sizem\exec + \sizeuei\exec = O((1+\sizep{\exec})\cdot\size{\code})$.
\end{corollary}
\begin{proofatend}
combining \refcoro{lazy-useful-bound1} with \reflemma{heap-bound}.
\end{proofatend}

Finally, we obtain the main result of the paper.

\begin{theorem}[Useful Implementation]\label{th:usefulimpl}\hfill
 \begin{enumerate}
  \item \emph{Low-Level Bilinear Implementation}: a $\togenlu$-derivation $\deriv$ is implementable on RAM in $O((1+\size\deriv)\cdot \size\tm)$  steps.
  \item \emph{Low + High Bilinear Implementation}: a $\tof$-derivation $\deriv$ is implementable on RAM in $O((1+\size\deriv)\cdot \size\tm)$ steps.
 \end{enumerate}
\end{theorem}


% \begin{theorem}
%  Let $\state$ be a state reached by an execution $\exec$ from an initial code $\code$. Then 
%  \begin{enumerate}
%   \item \emph{Bilinearity of Commutative Steps}: $\sizecom\exec = O(\sizep\exec \cdot \size\code)$.
%   \item \emph{Bilinearity of the Execution}: $\size\exec = O(\sizem\exec \cdot \size\code)$.
%  \end{enumerate}
% 
% 
% \end{theorem}



\begin{proofatend}
the proof follows from
\refthm{hlithm} applied to \refthm{lhli},
and \refth{lowlevelimplth} applied to \refth{lazy-uglam-refl-distillation} and \refcoro{useful-bound1}.
For the implementability of the steps we refer to the proof of \refth{preusefulimpl}.
\end{proofatend}


%\claudio{
%Considerazioni da fare da qualche parte:
%\begin{enumerate}
% \item I passi $\rename{}$ possono essere evitati per i passi $\tomachei$,
%   rilassando l'invariante di well-named in modo che chieda solamente che
%   nello scope di una variabile $\var$ non si ri-leghi $\var$. (Vedi commit
%   ritrattato in SVN).
% \item I passi $\tomachei$ possono essere implementati copiando un puntatore
%   e costano solo $O(1)$
% \item I passi $\tomachee$ debbono essere implementati copiando il termine
%   puntato e costano $O(\size{\code})$
% \item Il costo computazionale finale \`e dato dalla somma del costo dei
%   moltiplicativi (ognuno \`e $O(1)$), degli esponenziali interni
%   (ognuno \`e $O(1)$), di quelli esterni (ognuno \`e $O(\size{code})$)
%   e dei commutativi (ognuno \`e $O(1)$, ma sono in numero bilineare),
%   ma nuovamente solo sugli esterni.
%\end{enumerate}
%}


==> useful-machine.tex <==
% !TEX root = main.tex

\section{\fast\ \glamour}\label{sect:lazyglamour}
\begin{atend}\section{Proofs Omitted From \refsect{lazyglamour}\\ (\fast\ \glamour)}\end{atend}
\begin{atend}
The aim of this section is to prove \refth{lazy-uglam-refl-distillation}
($(\fast\ \glamour,\togenlu, \eqstruct, \decodefun)$ is a reflective explicit distillery) and the final result of the paper, \refth{usefulimpl}
(the useful implementation has bilinear low level and bilinear high level
complexity).

We follow closely the methodology of \refapp{glamour}. The first step is proving that the invariants of the machine holds.

\end{atend}
The \fast\ \glamour{} machine, in \reftab{useful-transitions}, behaves like the \glamour{} machine 
until the code is a variable $\var_1$ that is hereditarily bound in the global
environment to a value via the chain
$\esub{\var_1}{\var_2}^\alive \ldots \esub{\var_n}{\val}^\alive$. At this point the machine needs to traverse the chain
until it finds the final binding $\esub{\var_n}{\val}^\alive$, and then traverse
again the chain in the opposite direction replacing every
$\esub{\var_i}{\var_{i+1}}^\alive$ entry with $\esub{\var_i}{\val}^\alive$.

The forward traversal of the chain is implemented by a new commutative rule $\tomachcsix$
that pushes the variables encountered in the chain on a new machine component,
called the \emph{chain heap}. The backward traversal is driven by the next variable
popped from the heap, and it is implemented by a new exponential rule (the
\emph{chain} exponential rule, corresponding to that of the calculus). Most of the analyses performed on the
\glamour{} machine carry over to the \fast\ \glamour{} without modifications.

Every old grammar is as before, and heaps are defined by:
$$\begin{array}{rclllllllllll}
        \heap & \grameq & \heapempty \mid \heap\cons\var\\
\end{array}$$

\paragraph*{Decoding and Invariants} because of chain heaps and chain contexts, the decoding is involved. 

First of all, note that there is a correllation between the chain and the environment, as the variables of a chain heap $\heap = \var_1\cons\ldots\cons\var_n$ need to have corresponding entries $\esub{\var_i}{\var_{i+1}^\alive}$. More precisely, we will show that the following notion of compatibility is an invariant of the machine.

\begin{definition}[Compatibility Heap-Environment]
 Let $\genv$ be an environment and $\heap = \var_1 \cons \ldots \cons \var_n$ be a heap. We say that $\heap$ is \emph{compatible} with $\genv$ if 
 either $\heap$ is empty or $\esub{\var_i}{\var_{i+1}^\alive} \in \genv$ for $i < n$, $\esub{\var_n}{\var^\alive} \in \genv$, and $\esub{\var}{\stackitem^\alive} \in \genv$ for some $\stackitem^\alive$.
 \end{definition}

%A \emph{code} is a pure term, i.e. a term that does contain explicit
%substitutions. We will always overline codes to distinguish them from generic
%terms. A code $\code$ is \emph{initial} if it is a closed code.
%To reduce an initial code $\code$, $\code$ is injected into the initial
%state $\mac\epsilon\dumpempty\heapempty{\rename\code}\stempty$ where
%$\rename\code$ is a representative of the $\alpha$-equivalence class of
%$\code$ where all bound variables are pairwise distinct.

Given a state $\state = \mac\genv\dump\heap\code\stack$, the dump, the stack and the environment provide a shallow context $\tctx_\state  \defeq  \decgenvpx{\genv}{\decdumpp{\decstack}}$ that will be shown to be evaluable, as for the \glamour. 

If the chain heap $\heap$ is not empty, the current code $\code$ is somewhere in the middle of a chain inside the environment, and it is not apt to fill the state context $\tctx_\state$. The right code is the variable $\var_1$ starting the chain heap $\heap = \var_1\cons\ldots\cons\var_n$, \ie:

\begin{center}
$\begin{array}{rclllrcllllllll}
        \decodeheap{\heapempty}{\code} & \defeq & \code&&&
        \decodeheap{\var_1\cons\ldots\cons\var_n}{\code} & \defeq & \var_1
\end{array}$
\end{center}

Finally, a state decodes to a term as follows: $\decode{\state}  \defeq  \tctx_\state\ctxholep{\decodeheap{\heap}{\code}}$.

\begin{atend}
\begin{lemma}\label{l:heapprop1}
$ \decodeheap{\heap\cons\var}{\vartwo} = \decodeheap{\heap}{\var}$
\end{lemma}
\begin{IEEEproof}
by induction over $\heap$.
\end{IEEEproof}

\begin{lemma}[Contextual Decoding]\label{l:lazy-contextualdecoding}
$\decgenv$ is a substitution context; $\decdump$ and $\decstack$ are
shallow contexts without ES.
\end{lemma}
\begin{IEEEproof}
by induction over $\genv$, $\dump$ and $\stack$.
\end{IEEEproof}
\end{atend}


\begin{atend}
\begin{remark}
\label{rem:heap-comp}
if $\heap\cons\var$ is compatible with $\genv$, then also $\heap$ is compatible with $\genv$. 
\end{remark}
\end{atend}

\begin{lemma}[\fast\ \glamour\ Invariants]\label{l:lazy-uglaminvariants} % \reflemmap{lazy-uglaminvariants}{eval}
	Let $\state = \mac{\genv}{\dump}{\heap}{\codetwo}{\stack}$ be a state reachable from an initial code $\code$. 
	\begin{enumerate}
		\item \emph{Closure}:\label{p:lazy-uglaminvariants-closure} $\state$ is closed and $\state$ is well named;
		\item \emph{Value}:\label{p:lazy-uglaminvariants-value} values in components of $\state$ are sub-terms of $\code$;
		\item \emph{\Fireball}:\label{p:lazy-uglaminvariants-fireball} $\relunf\code{\decgenv}$ is a fireball (of kind $\lab$) for every code $\code^\lab$ in $\stack$ and $\genv$;
		\item \emph{Evaluability}:\label{p:lazy-uglaminvariants-eval} $\decode\genv$, $\relunf{\decdump}{\decode\genv}$, $\relunf{\decstack}{\decode\genv}$, and $\tctx_\state$ are evaluable cont.;

		\item \emph{Environment Size}:\label{p:lazy-uglaminvariants-size} the length of the global environment $\genv$ is
bound by $\sizem\exec$.
                \item \emph{Compatible Heap}:\label{p:lazy-uglaminvariants-heap} if $\heap \neq \heapempty$ then the stack is not empty, $\codetwo = \var$, and $\heap$ is compatible with $\genv$.
	\end{enumerate}
\end{lemma}

\begin{proofatend}
by induction over the length of the execution.
The base case holds because $\code$ is initial.
The inductive step is by cases over the kind of transition.
All the verifications are trivial. \refpoint{lazy-uglaminvariants-eval} is proved as in the non-optimized case (see \reflemma{uglaminvariants}, page \pageref{l:uglaminvariants}).
\end{proofatend}

We need additional decodings to retrieve the chain-starting context $\pevctx$ in the side-condition of $\togenfec$ rule, that---unsurprisingly---is given by the chain heap. Let $\state = \mac{\genv}{\dump}{\heap\cons\vartwo}{\code}{\stack}$ be a state s.t. $\heap\cons\vartwo$ is compatible with $\genv$. Note that compatibility gives $\genv = \genv_1\esub\vartwo{\herval\code}\genv_2$. Define the chain context $\psctx{\state}$ and the substitution context $\ssctx{\state}$ as:
\begin{center}
$\begin{array}{lclllllllllll}
        \psctx{\state} & \defeq & 
        \decgenvpx{\genv_1}{\decdumpp{\decstackp{\decheapp\vartwo}}}\esub\vartwo\ctxhole&&&

	\ssctx{\state} & \defeq & 
        \decode{\genv_2}        
\end{array}$
\end{center}

The first point of the following lemma guarantees that $\psctx{\state}$ and $\ssctx{\state}$ are well defined. The second point proves that filling $\ssctxp{\state}{\psctx{\state}}$ with the current term gives exactly the decoding of the state $\decode\state = \tctx_\state\ctxholep{\decheapp\vartwo}$, and that moreover the chain starts exaclty on the evaluable context given by the state, \ie\ that $\tctx_\state = \ssctxp{\state}{\tpctx{\psctx{\state}}\var} $.
 
\begin{lemma}[Heaps and Contexts]\label{l:heap-contexts}
	Let $\state = \mac{\genv}{\dump}{\heap\cons\vartwo}{\var}{\stack}$ be a state s.t. $\heap\cons\vartwo$ is compatible with $\genv$. Then:
	\begin{enumerate}
		\item $\ssctx{\state}$ is a substitution context and $\psctx{\state}$ is a chain context		
		\item s. t. $\decode\state = \tctx_\state\ctxholep{\decheapp\vartwo} = \ssctxp{\state}{\psctxp{\state}\var}$ with $\tctx_\state = \ssctxp{\state}{\tpctx{\psctx{\state}}\var} $
	\end{enumerate}
\end{lemma}

\begin{proofatend}
	the first point is trivial, we prove the other two. By induction on the length $k$ of $\heap$. Cases:
	 \begin{itemize}
	  \item \empty{$\heap$ is empty}, \ie\ $\heap=\heapempty$. By \reflemmap{lazy-uglaminvariants}{heap} we have $\genv \defeq \genv_1\esub\vartwo{\herval\var}\genv_2$. Let also $\tctx \defeq \decgenvp{\decdumpp{\decstack}}$. We have $ \decode\state =  \decgenvp{\decdumpp{\decstackp{\decheappp\vartwo{\heapempty\cons\vartwo}}}} = \tctxp{\decheappp\vartwo{\heapempty\cons\vartwo}}$ and
	 \begin{enumerate}
	 \item $\ssctx{\state} = \decode{\genv_2}$ and $\psctx{\state} = \decgenvpx{\genv_1}{\decdumpp{\decstackp{\vartwo}}}\esub\vartwo\ctxhole$, that (by \reflemma{lazy-contextualdecoding}) has the form $\tctxp\vartwo\esub\vartwo\ictx$, and so it is a chain context,
	 
	 \item Now, 
	 \begin{center}$\begin{array}{ll}
	 \decode\state & =\\
	 \tctx_\state\ctxholep{\decheappp\vartwo{\heapempty\cons\vartwo}} & = \\
         \decgenvp{\decdumpp{\decstackp{\decheappp\vartwo{\heapempty\cons\vartwo}}}} & =\\ 
	 \decgenvp{\decdumpp{\decstackp{\vartwo}}} & =\\
	 \decgenvpx{\genv_1\esub\vartwo{\herval\var}\genv_2}{\decdumpp{\decstackp{\vartwo}}} & =\\
	 \decgenvpx{\genv_2}{\decgenvpx{\genv_1}{\decdumpp{\decstackp{\vartwo}}}\esub\vartwo\var} & =\\
	 \ssctxp{\state}{\decgenvpx{\genv_1}{\decdumpp{\decstackp{\vartwo}}}\esub\vartwo\var} & =\\
         \ssctxp{\state}{\psctxp{\state}\var} 
	 \end{array}$\end{center}
	 
	 and
	 
	 \begin{center}$\begin{array}{ll}
	 \ssctxp{\state}{\tpctx{\psctx{\state}}\var}  & =\\
         \ssctxp{\state}{\tpctx{\decgenvpx{\genv_1}{\decdumpp{\decstackp{\vartwo}}}\esub\vartwo\ctxhole}\var} & = \\
	 \ssctxp{\state}{\decgenvpx{\genv_1}{\decdumpp{\decstack}}\esub\vartwo\var} & =\\ 
	 \decgenvpx{\genv_2}{\decgenvpx{\genv_1}{\decdumpp{\decstack}}\esub\vartwo\var} & =\\ 
	 \decgenvpx{\genv_1\esub\vartwo{\herval\var}\genv_2}{\decdumpp{\decstack}}& =\\
	 \decgenvpx{\genv}{\decdumpp{\decstack}} &=\\
         \tctx_\state\\
	 \end{array}$\end{center}
	 \end{enumerate}
	 
	 \item \empty{Non-empty}, \ie\ $\heap = \heaptwo\cons\varthree$. By \reflemmap{lazy-uglaminvariants}{heap} we have $\genv = \genv_1\esub\varthree{\herval\vartwo}\genv_2\esub\vartwo{\herval\var}\genv_3$ and $\tctx \defeq \decgenvp{\decdumpp{\decstack}}$, so that $\decode\state = \decgenvp{\decdumpp{\decstackp{\decheappp\vartwo{\heaptwo\cons\varthree\cons\vartwo}}}} = \tctxp{\decheappp\vartwo{\heaptwo\cons\varthree\cons\vartwo}}$. Note that by \refrem{heap-comp} we can apply the \ih\ to the state $\statetwo = \mac{\genv}{\dump}{\heaptwo\cons\varthree}{\vartwo}{\stack}$, and we will do it in the following points.
	 
	 Now,
	 \begin{enumerate}
	 \item $\ssctx{\state} = \decode{\genv_3}$ and for $\psctx{\state}$, note that we have $$\psctx\statetwo = \decgenvpx{\genv_1}{\decdumpp{\decstackp{\decheappp\vartwo{\heaptwo\cons\varthree}}}}\esub\varthree\ctxhole$$ and that by \ih\ $\psctx\statetwo$ is a chain context. Then
	 
	 \begin{center}$\begin{array}{lll}
	 \psctx{\state} & =\\
         \decgenvpx{\genv_1\esub\varthree{\herval\vartwo}\genv_2}{\decdumpp{\decstackp{\decheappp\vartwo{\heaptwo\cons\varthree}}}}\esub\vartwo\ctxhole & =\\
	 \decgenvpx{\genv_2}{\decgenvpx{\genv_1}{\decdumpp{\decstackp{\decheappp\vartwo{\heaptwo\cons\varthree}}}}\esub\varthree\vartwo}\esub\vartwo\ctxhole & =\\
         \decgenvpx{\genv_2}{\psctxp\statetwo\vartwo}\esub\vartwo\ctxhole
	 \end{array}$\end{center}
	 
	 and so $\psctx{\state}$ is a chain context.
	 
	 
	 \item Note that $\ssctx\statetwo = \decode{\genv_2\esub\vartwo{\herval\var}\genv_3}$, and so
	 \begin{center}$\begin{array}{lll}
	  \ssctxp{\state}{\psctxp{\state}\var} & =\\
	    \decgenvpx{\genv_3}{\decgenvpx{\genv_2} {\psctxp\statetwo\vartwo}\esub\vartwo\var} & =\\
	   \decgenvpx{\genv_2\esub\vartwo{\herval\var}\genv_3}{\psctxp\statetwo\vartwo} & =\\
	   \ssctxp\statetwo{\psctxp\statetwo\vartwo} & =_{\ih}\\
          \decode\state
	 \end{array}$\end{center}
	 
	 Then note that 
	 \begin{center}$\begin{array}{lll}
	 \tpctx{\psctx{\state}}\var  & =\\
         \tpctx{\decgenvpx{\genv_2}{\psctxp\statetwo\vartwo}\esub\vartwo\ctxhole}{\var} & =\\
	 \tpctx{\decgenvpx{\genv_2}{\psctx\statetwo}}\vartwo\esub\vartwo\var & =\\
         \decgenvpx{\genv_2}{\tpctx{\psctx\statetwo}\vartwo}\esub\vartwo\var
	 \end{array}$\end{center}
	 
	 Now we conclude with
	 \begin{center}$\begin{array}{lll}
	 \ssctxp{\state}{\tpctx{\psctx{\state}}\var}  & =\\
	 \decgenvpx{\genv_3}{\tpctx{\psctx{\state}}\var}  & =\\
	 \decgenvpx{\genv_3}{\decgenvpx{\genv_2}{\tpctx{\psctx\statetwo}\vartwo}\esub\vartwo\var} & = \\
	 \decgenvpx{\genv_2\esub\vartwo{\herval\var}\genv_3}{\tpctx{\psctx\statetwo}\vartwo} & = \\
	 \ssctxp\statetwo{\tpctx{\psctx\statetwo}\vartwo} & =_{\ih}\\
         \tctx_{\statetwo} & = \\
         \tctx_{\state}\\
	 \end{array}$\end{center}
	 \end{enumerate}
	 \end{itemize}
\end{proofatend}

We can now sum up.

\begin{atend}
\begin{lemma}[Explicit \glamour\ Distillation]\label{l:lazy-uglam-distillation}
	Let $\state$ be a reachable state. Then:
		\begin{enumerate}
		\item \emph{Commutative}: if $\state\tomachcp{_{1,2,3,4,5}}\statetwo$ then $\decode\state = \decode\statetwo$;
		\item \emph{Multiplicative}: if $\state\tomachum\statetwo$ then $\decode\state\togenum\eqstruct\decode\statetwo$;
		\item \emph{Shallow Exponential}: if $\state\tomachee\statetwo$ then $\decode\state\togenluee\decode\statetwo$;
		\item \emph{Chain Exponential}: if $\state\tomachei\statetwo$ then $\decode\state\togenluei\decode\statetwo$.
	\end{enumerate}
\end{lemma}

\begin{IEEEproof}
we list the transition in the order they appear in the definition of the machine.
\begin{itemize}
\item
Case
     $\mac{\genv}{\dump}{\heapempty}{\code\codetwo}{\stack}
     \tomachcone
     \mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\codetwo}{\stempty}$:
 $$\begin{array}{ll}
     \decode{\mac{\genv}{\dump}{\heapempty}{\code\codetwo}{\stack}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{(\code\codetwo)}}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\codetwo}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\ctxholep{\codetwo}}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\codetwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\codetwo}{\stempty}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\decodeheap{\heapempty}{\codetwo}}{\stempty}}}
     &=\\
     \decode{\mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\codetwo}{\stempty}}
 \end{array}$$

\item
Case 
     $\mac{\genv}{\dump}{\heapempty}{\la\var\code}{\stackitem^\lab\cons\stack}
     \tomachom
     \mac{\genv\esub\var{\stackitem^\lab}}{\dump}{\heapempty}{\code}{\stack}$:
 $$\begin{array}{ll}
     \decode{\mac{\genv}{\dump}{\heapempty}{\la\var\code}{\stackitem^\lab\cons\stack}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\la\var\code}}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\la\var\code}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{(\la\var\code)\decode{\stackitem}}{\stack}}}
     &\togenum\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\esub{\var}{\decode{\stackitem}}}{\stack}}}
     &\eqstruct\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{\stack}}\esub\var{\stackitem}}
     &=\\
     \decgenvpx{\genv\esub\var{\stackitem^\lab}}{\decodep{\dump}{\decodestack{\code}{\stack}}}
      &=\\
     \decgenvpx{\genv\esub\var{\stackitem^\lab}}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\code}}{\stack}}}
     &=\\
     \decode{\mac{\genv\esub\var{\stackitem^\lab}}{\dump}{\heapempty}{\code}{\stack}}
 \end{array}$$
The multiplicative step is justified by \reflemmap{lazy-uglaminvariants}{eval} and \reflemmap{lazy-uglaminvariants}{fireball}. The bisimulation step is justified by \reflemma{ev-comm-struct}.



\item
Case
     $$\mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\const}{\stacktwo}
     \tomachctwo
     \mac{\genv}{\dump}{\heapempty}{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}$$
We have
 $$\begin{array}{ll}
     \decode{\mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\const}{\stacktwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\decodeheap{\heapempty}{\decode{\const}}}{\stacktwo}}}
      &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\decode{\const}}{\stacktwo}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code\decodestack{\const}{\stacktwo}}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\code}}{\pair{\const}{\stacktwo}^\dead\cons\stack}}}
     &=\\
     \decode{\mac{\genv}{\dump}{\heapempty}{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}}
 \end{array}$$

\item
Case
     $$\begin{array}{l}\mac{\genv_1\esub\var{\stackitem^\dead}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stacktwo}
     \tomachcthree\\
     \mac{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump}{\heapempty}{\code}{\pair{\var}{\stacktwo}^\dead\cons\stack}\end{array}$$
We have
 $$\begin{array}{ll}
     \decode{\mac{\genv_1\esub\var{\stackitem^\dead}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stacktwo}}
     &=\\
     \ldots&\\
     \decode{\mac{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump}{\heapempty}{\code}{\pair{\var}{\stacktwo}^\dead\cons\stack}}
 \end{array}$$
The proof is the one for the previous case $\tomachctwo$,
by replacing $\const$ with $\var$ and instantiating $\genv$ with
${\genv_1\esub\var{\phi^\dead}\genv_2}$.

\item
Case
     $$\mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\la\var\codetwo}{\stempty}
     \tomachcfour
     \mac{\genv}{\dump}{\heapempty}{\code}{(\la\var\codetwo)^\alive\cons\stack}$$
We have
 $$\begin{array}{ll}
     \decode{\mac{\genv}{\dump\cons\nfnst\code\stack}{\heapempty}{\la\var\codetwo}{\stempty}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\decodeheap{\heapempty}{\la\var\codetwo}}{\stempty}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\decodestack{\la\var\codetwo}{\stempty}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump\cons\nfnst\code\stack}{\la\var\codetwo}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code(\la\var\codetwo)}{\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\code}{(\la\var\codetwo)^\alive\cons\stack}}}
     &=\\
     \decgenvpx{\genv}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\code}}{(\la\var\codetwo)^\alive\cons\stack}}}
     &=\\
     \decode{\mac{\genv}{\dump}{\heapempty}{\code}{(\la\var\codetwo)^\alive\cons\stack}}
 \end{array}$$

\item
Case
     $$\begin{array}{l}\mac{\genv_1\esub\var{\codetwo^\alive}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stempty}
     \tomachcfive\\
     \mac{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump}{\heapempty}{\code}{\var^\alive\cons\stack}\end{array}$$
We have
 $$\begin{array}{ll}
     \decode{\mac{\genv_1\esub\var{\codetwo^\alive}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stempty}}
     &=\\
     \ldots&=\\
     \decode{\mac{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump}{\heapempty}{\code}{\var^\alive\cons\stack}}
 \end{array}$$
The proof is the one for the previous case $\tomachcfour$,
by replacing $(\la\var\codetwo)$ with $\var$ and instantiating
$\genv$ with ${\genv_1\esub\var{\herval{\codetwo}}\genv_2}$.

\item
Case
     $$\begin{array}{l}\mac{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\var}{\stackitem^\lab\cons\stack}
     \tomachee\\
     \mac{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\rename\codeval}{\stackitem^\lab\cons\stack}\end{array}$$
We have
 $$\begin{array}{lll}
     \decode{\mac{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\var}{\stackitem^\lab\cons\stack}}
     &=\\
     \decgenvpx{\genv_1\esub\var{\herval\codeval}\genv_2}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\var}}{\stackitem^\val\cons\stack}}}
       &=\\
     \decgenvpx{\genv_1\esub\var{\herval\codeval}\genv_2}{\decodep{\dump}{\decodestack{\var}{\stackitem^\val\cons\stack}}}
     &\togenluee & \mbox{(by \reflemmaeqp{lazy-uglaminvariants}{eval})}\\
     \decgenvpx{\genv_1\esub\var{\herval\codeval}\genv_2}{\decodep{\dump}{\decodestack{\rename\codeval}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decgenvpx{\genv_1\esub\var{\herval\codeval}\genv_2}{\decodep{\dump}{\decodestack{\decodeheap{\heapempty}{\rename\codeval}}{\stackitem^\lab\cons\stack}}}
     &=\\
     \decode{\mac{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\rename\codeval}{\stackitem^\lab\cons\stack}}
 \end{array}$$

\item
Case
     $$\begin{array}{l}\mac{\genv_1\esub\var{\herval{\vartwo}}\genv_2}{\dump}{\heap}{\var}{\stackitem^\lab\cons\stack}
     \tomachcsix\\
     \mac{\genv_1\esub\var{\herval\vartwo}\genv_2}{\dump}{\heap\cons\var}{\vartwo}{\stackitem^\lab\cons\stack}\end{array}$$
 $$\begin{array}{ll}
   \decode{\mac{\genv_1\esub\var{\herval{\vartwo}}\genv_2}{\dump}{\heap}{\var}{\stackitem^\lab\cons\stack}}
   &=\\
   \decgenvpx{\genv_1\esub\var{\herval{\vartwo}}\genv_2}{\decodep{\dump}{\decodestack{\decodeheap{\heap}{\var}}{\stackitem^\lab\cons\stack}}}
   &=_\reflemmaeq{heapprop1}\\
   \decgenvpx{\genv_1\esub\var{\herval\vartwo}\genv_2}{\decodep{\dump}{\decodestack{\decodeheap{\heap\cons\var}{\vartwo}}{\stackitem^\lab\cons\stack}}}
   &=\\
   \decode{\mac{\genv_1\esub\var{\herval\vartwo}\genv_2}{\dump}{\heap\cons\var}{\vartwo}{\stackitem^\lab\cons\stack}}
 \end{array}$$

\item
Case
     $\statetwo \defeq \mac{\genv^\bullet}{\dump}{\heap\cons\vartwo}{\var}{\stackitem^\lab\cons\stack}
     \tomachei
     \mac{\genv^\circ}{\dump}{\heap}{\vartwo}{\stackitem^\lab\cons\stack} = \state$, where $\genv^\bullet = \genv_1\esub\vartwo{\herval\var}\genv_2\esub\var{\herval\codevalp}\genv_3$, and 
     $\genv^\circ = \genv_1\esub\vartwo{\herval{\mbox{$\rename\codevalp$}}}\genv_2\esub\var{\herval\codeval}\genv_3$. Note that we have:
     \begin{enumerate}
      \item $\ssctx{\statetwo,\vartwo} = \decode{\genv_2\esub\var{\herval\codevalp}\genv_3}$
      \item $\psctx{\statetwo,\vartwo} = \decgenvpx{\genv_1}{\decodep{\dump}{\decodestack{\decodeheap{\heap}{\vartwo}}{\stackitem^\val\cons\stack}}}\esub\vartwo\ctxhole $
     \end{enumerate}
Then,
 $$\begin{array}{ll}
     \decode{\mac{\genv^\bullet}{\dump}{\heap\cons\vartwo}{\var}{\stackitem^\lab\cons\stack}}
     &=\\
     \decgenvpx{\genv^\bullet}{\decodep{\dump}{\decodestack{\decodeheap{\heap\cons\vartwo}{\var}}{\stackitem^\val\cons\stack}}}
     &=\\
     \decgenvpx{\genv^\bullet}{\decodep{\dump}{\decodestack{\decodeheap{\heap}{\vartwo}}{\stackitem^\val\cons\stack}}}
     &=_\reflemmaeq{heap-contexts} \\
     \ssctxp{\statetwo,\vartwo}{\psctxp{\statetwo,\vartwo}\var}
     &=\\
     \decgenvpx{\genv_2\esub\var{\herval\codevalp}\genv_3}{\psctxp{\statetwo,\vartwo}\var}
     &=\\
     \decgenvpx{\genv_3}{\decgenvpx{\genv_2}{{\psctxp{\statetwo,\vartwo}\var}}\esub\var{\codevalp}}
     & \togenluei \\
     \decgenvpx{\genv_3}{\decgenvpx{\genv_2}{{\psctxp{\statetwo,\vartwo}{\rename\codevalp}}}\esub\var{\codevalp}}
     & = \\
     \decgenvpx{\genv_3}{\decgenvpx{\genv_2}{{\decgenvpx{\genv_1}{\decodep{\dump}{\decodestack{\decodeheap{\heap}{\vartwo}}{\stackitem^\val\cons\stack}}}\esub\vartwo{\rename\codevalp}}}\esub\var{\codevalp}}
     & = \\
     \decgenvpx{\genv^\circ}{\decodep{\dump}{\decodestack{\decodeheap{\heap}{\vartwo}}{\stackitem^\val\cons\stack}}}
     & =\\
     \decode{\mac{\genv^\circ}{\dump}{\heap}{\vartwo}{\stackitem^\lab\cons\stack}}     
 \end{array}$$
 The chain exponential step is justified because 
 \begin{enumerate}
  \item $\heap\cons\vartwo$ is compatible with $\genv^\bullet$, and so we can apply \reflemmaeq{heap-contexts}, obtaining $\ssctxp{\statetwo,\vartwo}{\tpctx{\psctx{\statetwo,\vartwo}}\var} = \decgenvpx{\genv^\bullet}{\decdumpp{\decode{\stackitem^\lab\cons\stack}}}$ 
  \item \reflemmap{lazy-uglaminvariants}{eval} guarantees that such a context---which is the context in the side-condition of the rule--- is evaluable. It is also obviously applicative (because the stack has the form $\stackitem^\lab\cons\stack$).\qedhere
 \end{enumerate}

\end{itemize}
\end{IEEEproof}

\begin{lemma}[Determinism]\label{l:lazy-uglam-deterministic} The reduction relation $\togen$ is deterministic.
\end{lemma}
\begin{IEEEproof}
a simple inspection of the reduction rules shows no critical pairs.
\end{IEEEproof}

\begin{lemma}[Progress]\label{l:lazyprogress} if $\state$ is reachable, $\admnf{\state}=\state$ and $\decode\state\togenx\tm$ with $\mathtt{x}\in\set{\lsym\usym\msym,\lsym\usym\esym\esym,\lsym\usym\esym\isym}$, then there exists $\statetwo$  such that $\state\tomachx\statetwo$, \ie, $\state$ is not final.
\end{lemma}
\begin{IEEEproof}
by \reflemma{lazy-uglam-deterministic} and \reflemma{lazy-uglam-distillation} it is sufficient to show that every reachable stuck state decodes to a normal form. The only stuck forms are:
\begin{itemize}
 \item \emph{Error states}. 
 \begin{enumerate}
  \item \emph{Problem with the heap}. $\mac{\genv}{\dump}{\heap\cons\vartwo}{\code}{\stack}$
   when $\code$ is not a variable bound in $\genv$ to a~$\stackitem^\alive$
   or $\stack$ is empty or $\vartwo$ is not bound to $\code$ in $\genv$.
   The state is not reachable because it would violate the
   invariant \reflemmap{lazy-uglaminvariants}{heap}.
   \item \emph{Problem with the environment}. The state is $\mac{\genv}{\dump}{\heap}{\var}{\stack}$ where $\var$ is not defined
  in $\genv$ or it is defined to be a $\herval\code$ where $\code$ is not
  a variable or a value.\\
   The state is not reachable because it would violate either the
   invariant in \reflemmap{lazy-uglaminvariants}{closure} or the invariant in
   \reflemmap{lazy-uglaminvariants}{fireball}.
 \end{enumerate}
 

 \item \emph{Final states}. Cases:
 \begin{enumerate}
  \item \emph{The result is/unfolds to a value}. The state is $\mac{\genv}{\dumpempty}{\heapempty}{\code}{\stempty}$
   with $\code$ an abstraction or a variable bound in
   $\genv$ to a $\stackitem^\alive$.
   By \reflemma{contextualdecoding},
   $\decode{\mac{\genv}{\dumpempty}{\heapempty}{\code}{\stempty}} =
    \decgenvpx{\genv}{\code} = \sctxp\code$ for some $\sctx$.
   Note that $\unf{\sctxp\code} = \relunf\code\sctx$ is a \fireball, indeed if $\code$ is an abstraction it is given by \reflemma{es-answers-are-normal} and if it as a variable it is given by \reflemmap{lazy-uglaminvariants}{fireball}.
   Thus by \reflemma{lazy-useful-projection}, $\sctxp\code$ is normal.

  \item \emph{The result is/unfolds to a generalized constant}. The state is $\mac{\genv}{\dumpempty}{\heapempty}{\code}{\stack}$
   with $\code$ a constant $\const$ or a variable bound in $\genv$ to a $\stackitem^\dead$.\\
   By \reflemma{contextualdecoding},
   $\decode{\mac{\genv}{\dumpempty}{\heapempty}{\code}{\stack}} = \decgenvpx{\genv}{\decodestack{\code}{\stack}} = 
    \sctxp{\decodestack{\code}{\stack}}$ for some $\sctx$.
   Note that $\unf{\sctxp\code} = \relunf\code\sctx$ is a \fireball, indeed if $\code$ is a constant it is given by \reflemma{es-answers-are-normal} and if it as a variable it is given by \reflemmap{lazy-uglaminvariants}{fireball}.
   Thus by \reflemma{lazy-useful-projection}, $\sctxp\code$ is normal.\qedhere
  \end{enumerate}
\end{itemize}
\end{IEEEproof}

\end{atend}

\begin{theorem}[\fast\ \glamour\ Distillation]\label{th:lazy-uglam-refl-distillation}
	$(\mbox{\fast\ \glamour},\togenlu, \eqstruct, \decodefun)$ is a reflective explicit distillery. In particular, let $\state$ be a reachable state:
	\begin{enumerate}
		\item \emph{Commutative}: if $\state\tomachcp{_{1,2,3,4,5,6}}\statetwo$ then $\decode\state = \decode\statetwo$;
		\item \emph{Multiplicative}: if $\state\tomachom\statetwo$ then $\decode\state\togenlum\eqstruct\decode\statetwo$;
		\item \emph{Shallow Exponential}: if $\state\tomachee\statetwo$ then $\decode\state\togenluee\decode\statetwo$;
		\item \emph{Chain Exponential}: if $\state\tomachei\statetwo$ then $\decode\state\togenluei\decode\statetwo$.
	\end{enumerate}
\end{theorem}
\begin{proofatend}
the theorem follows from \reflemma{lazy-uglam-distillation}, \reflemma{lazy-uglam-deterministic} and \reflemma{lazyprogress}.
\end{proofatend}


==> useful.tex <==
% !TEX root = main.tex
\begin{table*}
\caption{Transitions of the \fast\ \glamour}
\label{tab:useful-transitions}
\centering
  ${\setlength{\arraycolsep}{1em}
  \begin{array}{c|c|c|c|ccc|c|c|c|c}
     \maca{\genv}{\dump}{\heapempty}{\code\codetwo}{\stack}
     &\tomachcone&
     \maca{\genv}{\dump\cons \nfnst\code\stack}{\heapempty}{\codetwo}{\stempty}\\
  	
     \maca{\genv}{\dump}{\heapempty}{\l\var.\code}{\stackitem^\lab\cons\stack}
     &\tomachom &
     \maca{\econs{\esub\var{\stackitem^\lab}}{\genv}}{\dump}{\heapempty}{\code}{\stack}\\

     \maca{\genv}{\dump\cons \nfnst\code\stack}{\heapempty}{\const}{\stacktwo}
     & \tomachctwo &
     \maca{\genv}{\dump}{\heapempty}{\code}{\pair{\const}{\stacktwo}^\dead\cons\stack}\\

     \maca{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stacktwo}
     & \tomachcthree &
     \maca{\genv_1\esub\var{\phi^\dead}\genv_2}{\dump}{\heapempty}{\code}{\pair{\var}{\stacktwo}^\dead\cons\stack}\\

     \maca{\genv}{\dump \cons \nfnst\code\stack}{\heapempty}{\l\var.\codetwo}{\stempty}
     & \tomachcfour &
     \maca{\genv}{\dump}{\heapempty}{\code}{\herval{(\l\var.\codetwo)}\cons\stack}\\
		
     \maca{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump\cons\nfnst\code\stack}{\heapempty}{\var}{\stempty}
     & \tomachcfive &
     \maca{\genv_1\esub\var{\herval{\codetwo}}\genv_2}{\dump}{\heapempty}{\code}{\herval{\var}\cons\stack}\\

     \maca{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\var}{\stackitem^\lab\cons\stack}
     & \tomachee &
     \maca{\genv_1\esub\var{\herval\codeval}\genv_2}{\dump}{\heapempty}{\rename{\codeval}}{\stackitem^\lab\cons\stack}\\

     \maca{\genv_1\esub\var{\herval{\vartwo}}\genv_2}{\dump}{\heap}{\var}{\stackitem^\lab\cons\stack}
     & \tomachcsix &
     \maca{\genv_1\esub\var{\herval\vartwo}\genv_2}{\dump}{\heap\cons\var}{\vartwo}{\stackitem^\lab\cons\stack}\\

     \maca{\genv^\bullet}{\dump}{\heap\cons\vartwo}{\var}{\stackitem^\lab\cons\stack}
     & \tomachei &
     \maca{\genv^\circ}{\dump}{\heap}{\vartwo}{\stackitem^\lab\cons\stack}

  	\end{array}}$

\begin{minipage}{14cm}
 ~\\with $\genv^\bullet \defeq \genv_1\esub\var{\herval\codeval}\genv_2\esub\vartwo{\herval\var}\genv_3$, $\genv^\circ \defeq \genv_1\esub\var{\herval\codeval}\genv_2\esub\vartwo{\herval{\mbox{$\rename{\codeval}$}}}\genv_3$, and 
where $\rename{\codeval}$ is any code $\alpha$-equivalent to $\codeval$ that preserves well-naming of the machine.
\end{minipage}
\end{table*}

\section{The \FFC}\label{sect:usefullazy}
\begin{atend}\section{Proofs Omitted From \refsect{usefullazy}\\ (Optimizing Useful Reduction:\\ \FFC\ and the \fast\ \glamour)}\end{atend}
In this section we start by analyzing why the \UsFC{} has a quadratic overhead. We then refine it, obtaining the \FFC, that we will prove to have only a linear overhead wrt the \FC. The optimization has to do with the order in which chains of useful substitutions are performed.
\begin{atend}
We prove %\reflemma{benone} and
\reflemma{pseudo-trunks} first; then we address \refthm{lhli} ($(\tof,\togenf)$ is a globally bounded high-level implementation system) and \refprop{lazy-useful-strong-bis} ($\tostruct$ is a Strong Bisimulation).

~
\end{atend}

\paragraph*{Analysis of Useful Substitution Chains}
in the \UsFC, whenever there is a situation like
$$(\var_1\gconst)\esub{\var_1}{\var_2} \ldots \esub{\var_{n-1}}{\var_{n}}\esub{\var_n}{\val}$$
the $\togenu$ strategy performs $n+1$ exponential steps $\togenue$ 
replacing $\var_1$ with $\var_2$, then $\var_2$ with $\var_3$, and so on, until $\val$ is finally substituted on the head
$$\begin{array}{rlll}
   (\var_n\gconst)\esub{\var_1}{\var_2} \ldots \esub{\var_{n-1}}{\var_{n}}\esub{\var_n}{\val} & \togenue\\ (\val\gconst)\esub{\var_1}{\var_2} \ldots \esub{\var_{n-1}}{\var_{n}}\esub{\var_n}{\val}
  \end{array}$$
and a multiplicative redex can be fired. Any later occurrence of $\var_1$ will
trigger the same chain of exponential steps again. Because the length $n$ of the
chain is bounded by the number of previous multiplicative steps (local bound property), the overall
complexity of the machine is quadratic in the number of multiplicative steps. %And such a bound can be easily achieved, by adapting examples in \cite{DBLP:conf/rta/AccattoliL12,DBLP:conf/wollic/AccattoliC14}.
In our previous work \cite{DBLP:conf/wollic/AccattoliC14}, we showed that to reduce the
complexity to linear it is enough to perform substitution steps in reverse order, modifying the chains while traversing them. The idea is that in the previous example one should rather have a smart reduction $\togenfe$ ($\osym$ stays for optimized, as $\usym$ is already used for useful reduction) following the chain of substitutions and performing:
$$\begin{array}{llll}
   (\var_1\gconst)\esub{\var_1}{\var_2} \ldots \esub{\var_{n-1}}{\var_{n}}\esub{\var_n}{\val} & \togenfe\\ 
   (\var_1\gconst)\esub{\var_1}{\var_2} \ldots \esub{\var_{n-1}}{\val}\esub{\var_n}{\val} & \togenfe\\
   \ldots\\
   (\var_1\gconst)\esub{\var_1}{\val} \ldots \esub{\var_{n-1}}{\val}\esub{\var_n}{\val} & \togenfe\\
   (\val\gconst)\esub{\var_1}{\val} \ldots \esub{\var_{n-1}}{\val}\esub{\var_n}{\val}\\
  \end{array}$$
Later occurrences of $\var_1$ will no longer trigger the chain, because it has been \emph{unchained} by traversing it the first time.

Unfortunately, introducing such an optimization for useful reduction is hard. In the shown example, that has a very simple form, it is quite easy to define what \emph{following the chain} means. For the distillation machinery to work, however, we need our rewriting rules to be stable by structural equivalence, whose action is a rearrangement of substitutions through the term structure. Then the substitutions $\esub{\var_i}{\var_{i+1}}$ of the example can be spread all over the term, interleaved by applications and other substitutions, and even nested one into the other (like in $\esub{\var_i}{\var_{i+1}\esub{\var_{i+1}}{\var_{i+2}}}$). This makes the specification of optimized useful reduction a quite technical affair. 
%The overall process still requires $n$ exponential steps, called chain, to get rid of renaming substitutions $\esub{\var_i}{\var_{i+1}}$, and one final exponential step, called shallow, to replace the code $\var_1$ with $\val$. All later occurrences of any $\var_i$, however, will only trigger one shallow exponential step, since a chain of length $m$ has been replaced by $m$ chains of length 1.

\paragraph*{Chain Contexts} reconsider a term like in the example, $(\var\gconst)\esub{\var_1}{\var_2}\esub{\var_2}{\var_3}\esub{\var_3}{\var_4}\esub{\var_4}{\val}$. We want the next step to substitute on $\var_4$ so we should give a status to the context $\pevctx \defeq (\var\gconst)\esub{\var_1}{\var_2}\esub{\var_2}{\var_3}\esub{\var_3}{\ctxhole}$. The problem is that $\pevctx$ can be deformed by structural equivalence $\eqstruct$ as 
$$\pevctxtwo \defeq (\var\esub{\var_1}{\var_2\esub{\var_2}{\var_3}}\gconst)\esub{\var_3}{\ctxhole}$$
and so this context has to be caught too. We specify these context in \reftab{useful-rewritingrules} as \emph{chain contexts} $\pevctx$, defined using the auxiliary notion of \emph{identity context} $\ictx$, that captures a simpler form of chain (note that both notions are not shallow).

Given a chain context $\pevctx$, we will need to retrieve the point where the chain started, \ie\ the shallow context isolating the variable at the left end of the chain ($\var_1$ in the example). We are now going to define an operation associating to every chain context its \emph{chain-starting (shallow) context}. To see the two as contexts of a same term, we need also to provide the sub-term that we will put in $\pevctx$ (that will always be a variable). The chain-starting context $\startctx\pevctx\var$ associated to the chain context $\pevctx$ (with respect to $\var$) is defined in \reftab{useful-rewritingrules}.

For our example $\pevctx \defeq (\var\gconst)\esub{\var_1}{\var_2}\esub{\var_2}{\var_3}\esub{\var_3}{\ctxhole}$ we have  $\startctx{\pevctx}{\var_4} = (\ctxhole\gconst)\esub{\var_1}{\var_2}\esub{\var_2}{\var_3}\esub{\var_3}{\var_4}$, as expected.

\begin{atend}
%How can we be sure that we captured the right notion of chain and chain-starting context? First of all, chain contexts have to be stable by $\eqstruct$. 
%
%\begin{lemma}[Chains are Stable by $\eqstruct$]\label{l:benone}
% If $\pevctxp\var \eqstruct \tm$ then there is $\pevctxtwo$ s.t. $\tm = \pevctxtwop\var$ and $\tpctx\pevctx\var\eqstruct\tpctx\pevctxtwo\var$.
%\end{lemma}
%
%\begin{IEEEproof}
% \ben{to do}.
%\end{IEEEproof}

For chain-starting contexts $\startctx\pevctx\var$, we need prove that their hole is indeed the left end of the chain, with the help of a preliminary lemma.
 

\begin{lemma}
	\label{l:inert-ctx-unf}
	Let $\ictxp\var$ s.t. $\ictx$ does not capture $\var$. Then $\unf{\ictxp\var} = \var$.
\end{lemma}

\begin{IEEEproof}
	by induction on $\ictx$. Cases:
	\begin{enumerate}
		\item \emph{Base $\ictx = \ctxhole$}. Then $\unf{\ictxp\var} = \unf\var = \var$.
		\item \emph{Inductive $\ictx = \ictxp\vartwo\esub\vartwo\ictxtwo$}. Then 
		$$\begin{array}{l}\unf{\ictxp\var} = \unf{\ictxp\vartwo\esub\vartwo{\ictxtwop\var}} = \unf{\ictxp\vartwo}\isub\vartwo{\unf{\ictxtwop\var}} =_{\ih}\\ \vartwo\isub\vartwo{\unf{\ictxtwop\var}} =_{\ih} \vartwo\isub\vartwo{\var} = \var\end{array}$$
		\item \emph{Closure $\ictx = \ictx\esub\vartwo\tm$}. Then 
		$$\unf{\ictxp\var} = \unf{\ictxp\var\esub\vartwo\tm} = \unf{\ictxp\var}\isub\vartwo{\unf\tm} =_{\ih} \var\isub\vartwo{\unf\tm} = \var$$
	\end{enumerate}
\end{IEEEproof}




\begin{lemma}
	\label{l:pseudo-trunks}
	Let $\pevctxp\var$ s.t. $\pevctx$ does not capture $\var$. Then there exists $\vartwo$ s.t. $\pevctxp\var = \tpctxp\pevctx\var\vartwo$ and $\relunf\vartwo{\tpctx\pevctx\var} = \var$.
\end{lemma}

\myproof{\begin{IEEEproof}
	by induction on $\pevctx$. Cases:
	\begin{enumerate}
		\item	\emph{Base, \ie\ $\pevctx = \tctxp\vartwo\esub{\vartwo}{\ictx}$}. Then 
		$$\pevctxp\var = \tctxp\vartwo\esub{\vartwo}{\ictxp\var} = \tpctxp{\tctxtwop\vartwo\esub{\vartwo}{\ictx}}{\var}\vartwo$$
		Now, $\relunf\vartwo{\tpctx\pevctx\var} = \relunf\vartwo{\tctx\esub{\vartwo}{\ictxp\var}} = \unf{\ictxp\var} =_{\reflemmaeq{inert-ctx-unf}} \var$
		
		\item	\emph{Inductive, \ie\ $\pevctx = \pevctxtwop\varthree\esub{\varthree}{\ictx}$}. Then 
		$$\begin{array}{ll}
                  \pevctxp\var &=\\
                  \pevctxtwop\varthree\esub{\varthree}{\ictxp\var} &=_{\ih}\\
                  \tpctxp{\pevctxtwo}\varthree\vartwo\esub{\varthree}{\ictxp\var} &=\\
                  \tpctxp{\pevctxtwop\varthree\esub{\varthree}{\ictx}}\var\vartwo\end{array}$$
		
		Now, 
		$$\begin{array}{ll}
                  \relunf\vartwo{\tpctx\pevctx\var} &=\\
                  \relunf\vartwo{\tpctx{\pevctxtwo}\varthree\esub{\varthree}{\ictxp\var}} &=\\
                  \relunf\vartwo{\tpctx{\pevctxtwo}\varthree}\isub{\varthree}{\unf{\ictxp\var}} &=_{\ih}\\
                  \varthree\isub{\varthree}{\unf{\ictxp\var}} = \unf{\ictxp\var} =_{\reflemmaeq{inert-ctx-unf}} \var\end{array}$$
		
		\item	\emph{Closure, \ie\ $\pevctx = \tctxtwop\pevctxtwo$}. Then 
		$$\pevctxp\var = \tctxtwop{\pevctxtwop\var} =_{\ih} \tctxtwop{\tpctxp{\pevctx}{\var}\vartwo} = \tpctxp{\tctxtwop\pevctx}{\var}\vartwo$$
		Now, $$\relunf\vartwo{\tpctx\pevctx\var} = \relunf\vartwo{\tctxtwop{\tpctx{\pevctx}{\var}}} =_{\reflemmaeqp{relunf-properties}{five}} \relunf{\relunf\vartwo{\tpctx{\pevctx}{\var}}}\tctxtwo =_{\ih} \relunf\var\tctxtwo = \var$$ because $\pevctx$, and thus $\tctxtwo$, does not capture $\var$.\qedhere
	\end{enumerate}
\end{IEEEproof}}
\end{atend}

\paragraph*{Rewriting Rules} the rules of the \FFC\ are in \reftab{useful-rewritingrules}. Note that the exponential rule splits in two, the ordinary \emph{shallow} case $\togenfes$ (now constrained to values) and the \emph{chain} case $\togenfec$ (where the new definition play a role). They could be merged, but for the complexity analysis and the relationship with the next machine is better to distinguish them. We use $\togenlue$ for $\togenluee\cup\togenluei$, and $\togenlu$ for $\togenlum\cup\togenlue$. Note the use of $\tpctx\pevctx\var$ in the third side condition. 

\subsection{Multiplicative vs Exponential Analysis} 
To prove that $\togenf$ implements $\tof$ with a global bound, and thus with a linear overhead, we need to show that the global number of $\togenfe$-steps in a $\togenf$-derivation is bound by the number of multiplicative steps. We need the following invariant.

\begin{lemma}[Subterm Invariant]
	\label{l:useful-subterm}
	Let $\tm$ be a $\l$-term and $\deriv:\tm\togen^*\tmtwo$. Then every value in $\tmtwo$ is a value in $\tm$.
\end{lemma}

\begin{proofatend}
by induction over the length of the derivation. A simple inspection of the
rewriting rules shows that all values in the result of a reduction step are
copies of values in the term being reduced.
\end{proofatend}

A substitution $\tm\esub\var\tmtwo$ is \emph{\basic}\ if $\tmtwo$ has the form $\sctxp\vartwo$. The \emph{basic size} $\sizeb\tm$ of $\tm$ is the number of its  basic substitutions.

\begin{lemma}[Steps and Basic Size]
	\label{l:steps-basic-size} % \reflemma{steps-basic-size}.\ref{steps-basic-size-one}
	\hfill
	\begin{enumerate}
		\item \label{p:steps-basic-size-one} If $\tm\togenluee\tmtwo$ then $\sizeb\tmtwo = \sizeb\tm$;
		\item \label{p:steps-basic-size-two} If $\tm\togenluei\tmtwo$ then $\sizeb\tm > 0$ and $\sizeb\tmtwo = \sizeb\tm - 1$;
		\item \label{p:steps-basic-size-three} If $\tm\togenlum\tmtwo$ then $\sizeb\tmtwo = \sizeb\tm$ or $\sizeb\tmtwo = \sizeb\tm +1$.
	\end{enumerate}
\end{lemma}

\begin{proofatend}
	using the sub-term property (\reflemma{useful-subterm}).
\end{proofatend}

\begin{lemma}
Let $\tm$ be initial and $\deriv:\tm\togenlu^*\tmtwo$. Then $\sizeb\tmtwo \leq \sizeum\deriv - \sizeuei\deriv$.
\end{lemma}

\begin{IEEEproof}
	by induction on $\size\deriv$. If $\size\deriv = 0$ the statement holds. If $\size\deriv>0$ consider the last step $\tmthree\togenlu\tmtwo$ of $\deriv$ and the prefix $\derivtwo:\tm\togenlu^*\tmthree$ of $\deriv$. By \ih, $\sizeb\tmthree \leq \sizeum\derivtwo - \sizeuei\derivtwo$. Cases of $\tmthree\togenlu\tmtwo$.\\ \emph{Shallow Exponential Step $\togenluee$}:
		$$\begin{array}{rllllll}
		\sizeb\tmtwo &\leq_{\reflemmaeqp{steps-basic-size}{one}}&
		 \sizeb\tmthree-1 &\\
		  &\leq_{\ih}&\sizeum\derivtwo - \sizeuei\derivtwo -1 &\\
		   &=&\sizeum\derivtwo - (\sizeuei\derivtwo +1) &=
		    &\sizeum\deriv - \sizeuei\deriv
		    \end{array}$$
 \emph{Chain Exponential Step $\togenluei$}:
		$$\sizeb\tmtwo =_{\reflemmaeqp{steps-basic-size}{two}} \sizeb\tmthree \leq_{\ih} \sizeum\derivtwo - \sizeuei\derivtwo =  \sizeum\deriv - \sizeuei\deriv$$
 \emph{Multiplicative Step $\togenlum$}:
		$$\begin{array}{lllllll}
		\sizeb\tmtwo & \leq_{\reflemmaeqp{steps-basic-size}{three}}&
		\sizeb\tmthree+1 \\
		& \leq_{\ih} & \sizeum \derivtwo - \sizeuei\derivtwo +1 \\
		& = & \derivtwo +1 - \sizeuei\derivtwo &= & \sizeum\deriv - \sizeuei\deriv\quad\qedhere\end{array}$$
\end{IEEEproof}


\begin{corollary}[Linear Bound on Chain Exponential Steps]
	\label{coro:linear-bound-internal-exp}
	Let $\tm$ be initial and $\deriv:\tm\togenlu^*\tmtwo$. Then $\sizeuei\deriv \leq \sizeum\deriv$.
\end{corollary}

Next, we bound shallow steps.

\begin{lemma}[Linear Bound on Shallow Exponential Steps]
	\label{l:linear-bound-external-exp}
	Let $\tm$ be initial and $\deriv:\tm\togenlu^*\tmtwo$. Then $\sizeuee\deriv \leq \sizeum\deriv$.
\end{lemma}

\begin{IEEEproof}
	first note that if $\tm\togenluee\tmtwo$ then $\tmtwo\togenlum\tmthree$, because by definition $\togenluee$ can fire only if it creates a $\togenlum$-redex. Such a fact and determinism of $\togenlu$ together imply $\sizeuee\deriv \leq \sizeum\deriv+1$, because every $\togenluee$ step is matched by the eventual $\togenlum$ steps that follows it immediately. However, note that in $\tm$ there are no explicit substitutions so that the first step is necessarily an unmatched $\togenlum$ step. Thus $\sizeuee\deriv \leq \sizeum\deriv$.
\end{IEEEproof}

\begin{theorem}[Linear Bound on Exponential Steps]
\label{tm:linear-exponentials}
	Let $\tm$ be initial and $\deriv:\tm\togenlu^*\tmtwo$. Then $\sizeoe\deriv \leq 2\cdot \sizeum\deriv$.
\end{theorem}

\begin{IEEEproof}
	by definition, $\sizeoe{\deriv} = \sizeuei{\deriv} + \sizeuee{\deriv}$. By \refcoro{linear-bound-internal-exp}, $\sizeuei{\deriv} \leq \sizeum{\deriv}$ and by \reflemma{linear-bound-external-exp} $\sizeuee{\deriv} \leq \sizeum{\deriv}$, and so $\sizeoe\deriv \leq 2\cdot \sizeum\deriv$.
\end{IEEEproof}

We presented the interesting bit of the proof of our improved high-level implementation theorem, which follows. The remaining details are in the appendix.

\begin{atend}
\input{\proofspath/unchaining-normal-forms-and-determinism}
\end{atend}

\begin{theorem}[Linear High-Level Implementation]\label{thm:lhli}
	$(\tof,\togenlu)$ is a globally bounded high-level implementation system, and so it has a linear overhead wrt $\tof$.
\end{theorem}

\begin{proofatend}
the pair $(\tof,\togenlu)$ is an high-level implementation system because of
\reflemma{lazy-useful-determinism},
\reflemma{lazy-useful-projection} and
\refcoro{lazy-useful-nfs-unfold-to-nfs-useful}.
It is also globally bounded because we already proved the global linear bound
on exponential steps (\reftm{linear-exponentials}).
\end{proofatend}


%\begin{lemma}[Substitution Sequences]
%\label{l:inert-length}
%If $\tm$ is not $\togenue$-normal then there are $\tmtwo$ and $k$ s.t. $\tm\togenluei^k\togenluee\togenlum\tmtwo$ and $k\leq\sizeb\tm$.
%\end{lemma}
%
%\begin{proofatend}
%	By induction on $\sizeb\tm$. 
%	\begin{enumerate}
%		\item \emph{No Basic Substitution}, \ie\ $\sizeb\tm = 0$. Then by \reflemma{steps-basic-size}.\ref{p:steps-basic-size-one} (and determinism) $\tm\togenluee\tmthree$ for some $\tmthree$. By definition of $\togenluee$ (and determinism) this step creates a multiplicative redex, and so $\tm\togenluee\togenlum\tmtwo$ for some $\tmtwo$.
%		\item \emph{Some Basic Substitution}, \ie\ $\sizeb\tm > 0$. If $\tm\togenluee\tmthree$ for some $\tmthree$ then we reason as in the previous case. Otherwise, (by determinism) $\tm\togenluei\tmthree$ and by  \reflemma{steps-basic-size}.\ref{p:steps-basic-size-two} $\sizeb\tmthree = \sizeb\tm -1$. The \ih\ gives $\tmtwo$ and $k'$ s.t. $\tmthree\togenluei^{k'}\togenluee\togenlum\tmtwo$, with $k\geq\sizeb\tm -1$ and we conclude because $\tm\togenluei\tmthree\togenluei^{k'}\togenluee\togenlum\tmtwo$.
%	\end{enumerate} 
%\end{proofatend}

Last, the structural equivalence $\equiv$ is a strong bisimulation also for the \FFC.

\begin{proposition}[$\tostruct$ is a Strong Bisimulation]	
	\label{prop:lazy-useful-strong-bis}
	Let $\mathtt{x}\in\set{\osym\msym,\osym\msym\ssym, \osym\msym\csym}$. Then, $\tm\eqstruct\tmtwo$ and $\tm\togenx\tmp$ implies that there exists $\tmtwop$ such that $\tmtwo\togenx\tmtwop$ and $\tmp\eqstruct\tmtwop$.
\end{proposition}

\begin{proofatend}
omitted. All postponement proofs are similar and lengthy.
In \refssect{app-struct-eq} of the Appendix we proved the lemma for the \ShFC.
Other examples can be found in the long version of~\cite{DBLP:conf/icfp/AccattoliBM14}.
\end{proofatend}

